UDAPose: Unsupervised Domain Adaptation for Low-Light Human Pose Estimation

Low-visibility scenarios, such as low-light conditions, pose significant challenges to human pose estimation due to the scarcity of annotated low-light datasets and the loss of visual information under poor illumination. Recent domain adaptation techniques attempt to utilize well-lit labels by augmenting well-lit images to mimic low-light conditions. But handcrafted augmentations oversimplify noise patterns, while learning-based methods often fail to preserve high-frequency low-light characteristics, producing unrealistic images that lead pose models to generalize poorly to real low-light scenes. Moreover, recent pose estimators rely on image cues through image-to-keypoint cross-attention, but these cues become unreliable under low-light conditions. To address these issues, we propose Unsupervised Domain Adaptation for Pose Estimation (UDAPose), a novel framework that synthesizes low-light images and dynamically fuses visual cues with pose priors for improved pose estimation. Specifically, our synthesis method incorporates a Direct-Current-based High-Pass Filter (DHF) and a Low-light Characteristics Injection Module (LCIM) to inject high-frequency details from input low-light images, overcoming rigidity or the detail loss in existing approaches. Furthermore, we introduce a Dynamic Control of Attention (DCA) module that adaptively balances image cues with learned pose priors in the Transformer architecture. Experiments show that UDAPose outperforms state-of-the-art methods, with notable AP gains of 10.1 (56.4%) on the ExLPose-test hard set (LL-H) and 7.4 (31.4%) in cross-dataset validation on EHPT-XC. Code: https://github.com/Vision-and-Multimodal-Intelligence-Lab/UDAPose

==> camera_ver/main_paper_v1.tex <==
\begin{abstract}
%
Low-visibility scenarios, such as low-light conditions, pose significant challenges to human pose estimation due to the scarcity of annotated low-light datasets and the loss of visual information under poor illumination. 
%
Recent domain adaptation techniques attempt to utilize well-lit labels by augmenting well-lit images to mimic low-light conditions.
%
But handcrafted augmentations oversimplify noise patterns, while learning-based methods often fail to preserve high-frequency low-light characteristics, producing unrealistic images that lead pose models to generalize poorly to real low-light scenes.
%
Moreover, recent pose estimators rely on image cues through image-to-keypoint cross-attention, but these cues become unreliable under low-light conditions.
%
To address these issues, we propose Unsupervised Domain Adaptation for Pose Estimation (UDAPose), a novel framework that synthesizes low-light images and dynamically fuses visual cues with pose priors for improved pose estimation.
%
Specifically, our synthesis method incorporates a Direct-Current-based High-Pass Filter (DHF) and a Low-light Characteristics Injection Module (LCIM) to inject high-frequency details from input low-light images, overcoming rigidity or the detail loss in existing approaches.
%
Furthermore, we introduce a Dynamic Control of Attention (DCA) module that adaptively balances image cues with learned pose priors in the Transformer architecture.
%
Experiments show that UDAPose outperforms state-of-the-art methods, with notable AP gains of 10.1 (56.4\%) on the ExLPose-test hard set (LL-H) and 7.4 (31.4\%) in cross-dataset validation on EHPT-XC.
%
Code: \href{https://github.com/Vision-and-Multimodal-Intelligence-Lab/UDAPose}{VMIL/UDAPose}.
% \hl{leading to unrealistic appearances and thus limits the performance of a model trained on such data when applied to real low-light images.}\yihao{May be a little verbose. It can be shorter such as "learning-based methods often fail to preserve high-frequency low-light characteristics, resulting in unrealistic appearances and degraded performance on real low-light data."}
\end{abstract}




\section{Introduction}
\label{sec:intro}
%
\input{figures/fig_baseline_comp}
%
Human pose estimation is a foundational task in computer
vision, essential for many downstream applications~\cite{application-healthcare,application-traffic,application-sports2,application-ar,application-security,survey-application-2021}.
%
Existing methods~\cite{rw-poseur,purkrabek2025probpose,rw-swahr,LOGOCAP,grouppose,tan2024diffusionregpose}
and benchmark datasets~\cite{lin2014microsoft,li2019crowdpose,dataset-ochuman}
primarily focus on well-illuminated scenarios.
%
However, real-world scenarios often involve low-light conditions, which significantly degrade pose estimation performance~\cite{ExLPose_2023_CVPR,ehpt-xc} and result in safety risks~\cite{tesla-NHTSA}. 
%
A key challenge is the scarcity of real-world low-visibility datasets, as annotating such images is inherently difficult.
%
\citet{ExLPose_2023_CVPR} introduced a specialized camera system to capture paired well-lit and low-light images, transferring annotations from well-lit to low-light counterparts.
%
However, these artificially darkened images cannot fully replicate real
low-light conditions, limiting the generalization of models trained on them~\cite{li2021learning}.
%
Although event cameras~\cite{ehpt-xc} offer an alternative, they require specialized hardware and complex cross-modality alignment, which limits scalable deployment.


While paired data collection is impractical, an alternative approach is to apply low-light image enhancement methods~\cite{yang2023implicit,quadprior,cai2023retinexformer,feijoo2025darkir,jiang2024lightendiffusion}.
%
However, this recovery process is inherently ill-posed, as reconstructing missing visual details from severely degraded images is challenging and often leads to artifacts that negatively impact human pose estimation.\textbf{}
%
Instead of recovering lost details, domain-adaptive methods~\cite{ella-eccv,kim2022unified} take a different approach by synthesizing low-light images from well-lit ones to mimic low-visibility conditions.
%
This allows models to leverage existing well-lit annotations during training.
%
These methods typically rely on handcrafted augmentations~\cite{ella-eccv} or learning-based image-to-image translation~\cite{CycleGAN2017,cai2024enco,kim2023unsb} to bridge the domain gap.
%
However, their effectiveness depends on how well they replicate real low-light characteristics, which remains a significant and underexplored challenge.


Handcrafted augmentations often fail to replicate the complex characteristics of real low-light images.
%
For instance, ELLA~\cite{ella-eccv} applies Gaussian white noise to simulate low-light conditions. 
%
However, real low-light noise, such as photon noise, thermal noise, and quantization noise, is far more complex~\cite{wei2021physics}. 
%
% \edit{Moreover, rule-based augmentations lack flexibility, as they are designed for specific low-light conditions.}
Moreover, handcrafted augmentations exhibit limited flexibility and generalization, as they are tailored to specific low-light scenarios. 
%
Consequently, their deployment in novel environments, such as those involving different camera hardware or new datasets (e.g., EHPT-XC~\citep{ehpt-xc}), often results in suboptimal performance and requires extensive manual tuning.
%
Learning-based augmentations utilize unpaired image-to-image translation~\cite{CycleGAN2017, kim2023unsb, chung2024style} to adapt well-lit images to low-light conditions.
%
However, as shown in~\cref{fig:intro-baseline-gen-comp}, these methods fail to replicate realistic low-light characteristics. 
%
CycleGAN~\cite{CycleGAN2017} tends to overly darken images while introducing lighting artifacts, while StyleID~\cite{chung2024style} fails to generate realistic low-light noise.


Beyond the limitations of low-light data synthesis, the robustness of modern pose estimators themselves becomes a critical factor, particularly the recent one-stage architectures~\cite{edpose,grouppose,tan2024diffusionregpose}.
%
When visual cues are subtle or entirely absent, a robust model should leverage learned pose priors to infer keypoints hidden in darkness.
%
However, recent one-stage pose estimators~\cite{edpose,grouppose,tan2024diffusionregpose}, often built upon DETR-like architectures~\cite{DETR,deformable-detr}, utilize cross-attention to query image features and fuse them with pose priors via a direct residual connection. 
%
This rigid summation biases the fused representation toward image cues, even when the visual information is unreliable, particularly under low-light conditions.
%
Empirically, we observe that the model consistently emphasizes cross-attention visual features over pose-prior features under both well-lit and low-light conditions (see~\cref{fig:l2norm} for L2-norm comparisons).
%
Consequently, under poor illumination, noisy and unreliable visual features still contribute significantly compared to the pose priors, leading to unreliable human pose predictions, particularly for the low-visibility keypoints.
% \yihao{This sentence suggests that the previous method already considers pose priors, but it is not clear why this leads the model to heavily rely on image cues. Even though the next sentence attributes this to the rigid summation of image and prior features, the explanation is still not explicit. Perhaps we can soften the tone and clarify the mechanism, e.g., “we found that with rigid summation, the model tends to emphasize image cues regardless of their visibility.” After that, we could reference the quantitative results (L2-norm/eigen value)or visual examples to support this point."}


To overcome the above limitations, we propose UDAPose, a novel framework for unsupervised domain adaptation in human pose estimation.
%
Our framework employs Stable Diffusion (SD)~\cite{latentdiffusion} as a generative backbone to synthesize low-light images from well-lit ones.
%
By using unlabeled low-light images as references, UDAPose synthesizes augmentations that better reflect real low-light characteristics, outperforming existing approaches.
%
Our approach is highly practical, as collecting unlabeled low-light images is far easier than obtaining corresponding pose annotations.
%
To capture low-light characteristics from reference images, we introduce (1) Direct-Current-based High-Pass Filter (DHF), which extracts high-frequency low-light characteristics and (2) Low-Light Characteristics Injection Module (LCIM), which ensures that synthesized images retain complex low-light features of the reference images.
%
Unlike existing learning-based augmentations, UDAPose preserves essential low-light characteristics for human pose estimation, achieving significant performance gains.
%
A representative example is shown in the last column of~\cref{fig:intro-baseline-gen-comp}.


To address the vulnerability of pose estimation models under low-light conditions, we introduce the Dynamic Control of Attention (DCA) module. 
%
DCA adaptively controls the fusion weight between visual cues and pose priors, allowing the model to dynamically adjust the contributions from image features and learned human pose priors when visual information is degraded.
%
In summary, our contributions are as follows. 
\begin{itemize}
    \item 
    We propose UDAPose, an unsupervised domain adaptation framework that augments well-lit images to mimic low-light conditions and adaptively fuses visual cues with learned pose priors, achieving improved low-light human pose estimation without requiring low-light annotations.
    \item 
    We introduce the Direct-Current-based High-Pass-Filter (DHF) and Low-Light Characteristics Injection Module (LCIM), which preserve and inject high-frequency details to the synthesized low-light images.
    \item
    We propose Dynamic Control of Attention (DCA), which dynamically balances image cues with learned pose priors in the Transformer architecture, reducing the influence of noisy and unreliable visual cues in low-light scenarios. 
\end{itemize}
%
Experimental results show UDAPose surpasses existing methods, achieving a 10.1 AP (56.4\%) improvement on the low-light hard set (LL-H) of ExLPose-test and a 7.4 AP (31.4\%) improvement in cross-dataset evaluation on EHPT-XC, highlighting its robustness under low-light conditions.




\section{Related Work}
\label{sec:related}
%
\noindent\textbf{Human Pose Estimation}
Modern human pose estimation is primarily categorized into two mainstream paradigms: top-down and bottom-up. Top-down approaches~\cite{rw-poseur,wang2024locllm,purkrabek2025probpose} first detect individuals and subsequently estimate the pose for each one. In contrast, bottom-up approaches~\cite{DEKR2021,rw-swahr,LOGOCAP} first detect all body keypoints in the image and then assemble them into distinct person instances.
%
Recent advances, including one-stage unified detection-estimation frameworks~\cite{tian2019directpose,mao2021fcpose,shi2021inspose,xiao2022querypose,edpose,grouppose,tan2024diffusionregpose} and Vision Transformer-based models~\cite{rw-petr,xu2022vitpose,wang2024locllm,khirodkar2024sapiens}, have achieved remarkable accuracy. 
%
However, these models are trained and evaluated primarily on benchmarks with ideal lighting conditions~\cite{lin2014microsoft,li2019crowdpose,dataset-lsp,dataset-ochuman}. In particular, recent one-stage methods~\cite{edpose,grouppose,tan2024diffusionregpose} that rely on image cues become unreliable under low-light conditions.
%
Consequently, their performance degrades significantly in low-light scenarios~\cite{ExLPose_2023_CVPR,ehpt-xc}. 
%
While some works have explored domain adaptation~\cite{kim2022unified, peng2023source, raychaudhuri2023prior, cao2019cross, li2021synthetic, mu2020learning, han2022learning, jiang2021regressive, jin2022multibranch} or simple rule-based augmentations~\cite{ella-eccv}, they either lack specific designs for low-light characteristics or fail to synthesize realistic degradation. 
%
Methods requiring paired low-light and well-lit images~\cite{ExLPose_2023_CVPR}, or additional event camera data~\cite{ehpt-xc} are impractical due to the difficulty of collecting such data at scale and their limited scalability in deployment.

\noindent\textbf{Low-light Image Enhancement}
An intuitive approach for low-light pose estimation is to first apply a low-light image enhancement (LLIE) method as a pre-processing step. 
%
While deep learning techniques, including CNNs~\cite{moran2020deeplpf, sharma2021nighttime, wang2019underexposed}, GANs~\cite{huang2017arbitrary, jin2022unsupervised, jiang2021enlightengan, yang2023implicit}, Transformers~\cite{cai2023retinexformer,feijoo2025darkir}, and diffusion models~\cite{LLFlow, jiang2024lightendiffusion,quadprior}, have surpassed traditional methods like histogram equalization~\cite{celik2011contextual, cheng2004simple} and Retinex-based approaches~\cite{li2018structure, wang2013naturalness}, they still face significant challenges. 
%
These methods can introduce artifacts or fail to restore sufficient detail in extremely dark images, which in turn limits the performance of any subsequent pose estimation model.

\noindent\textbf{Unpaired Image-to-Image Translation}
Unpaired image-to-image (I2I) translation offers a promising direction for generating synthetic training data. 
%
Seminal works like CycleGAN~\cite{CycleGAN2017} enabled translation without paired data, a concept extended by style transfer methods like AdaIN~\cite{huang2017arbitrary}. 
%
More recently, diffusion-based models~\cite{kim2023unsb,chung2024style,xia2024diffusion,xia2024diffi2i} have demonstrated powerful capabilities in domain mapping. 
%
However, the primary objective of these generic I2I methods is to alter global appearance and texture. They are not specifically designed to synthesize the complex, non-uniform noise and structural degradation characteristic of low-light conditions, which is crucial for training a robust pose estimator. 
%
This distinction motivates our work on a specialized low-light augmentation strategy tailored for high-level vision tasks.
%
\input{figures/overall_arch}




\section{Method}
\label{sec:method}
%
\noindent\textbf{Overview} 
UDAPose is a novel unsupervised domain adaptation framework that synthesizes low-light images from well-lit ones and adaptively fuses visual cues with learned pose priors for robust human pose estimation. 
%
As illustrated in~\cref{fig:overall_arch}, our approach uses a pre-trained Stable Diffusion (SD) model to transfer scene structure from an annotated well-lit image while injecting low-light characteristics from an unlabeled reference image, enabling supervised pose training in the low-light conditions without requiring low-light annotations. 
%
We obtain the style-infused latent code $z_0$, which embeds the structure of the well-lit image $I_\text{WL}$ and the low-frequency style of the reference $I_\text{LL}$ following~\citet{chung2024style}.
%
During the decoding process, $z_0$ is decoded, where low-light noise patterns are injected through two key modules, DHF and LCIM.
%
The diffusion backbone is responsible for preserving the scene structure and low-frequency appearance from the well-lit image, while DHF and LCIM focus on injecting high-frequency low-light characteristics.
%
The obtained low-light images are then used as training data for our Transformer-based pose estimator, where our DCA module adaptively balances image cues and pose priors to mitigate unreliable visual information under low-light conditions.


\begin{comment}

We tackle the challenge of 2D human pose estimation in low-light conditions with UDAPose, a novel unsupervised domain adaptation framework. As shown in Figure~\ref{fig:overall_arch}, UDAPose leverages a pre-trained Stable Diffusion (SD) model~\cite{latentdiffusion} to synthesize a realistic low-light image $\hat{I}_{\rm LL}$. It achieves this by combining the structural content from an annotated well-lit image $I_{\rm WL}$ with the low-light characteristics of an unlabeled low-light reference image $I_{\rm LL}$. This approach enables the direct transfer of pose annotations from $I_{\rm WL}$ to $\hat{I}_{\rm LL}$, allowing \edit{fully}{} supervised training of a pose estimator \edit{in the low-light domain}{for low-light conditions}.


Our synthesis pipeline uses the frozen VAE encoder $\mathcal{E}$, decoder $\mathcal{D}$, and UNet denoising backbone of the SD model. The process consists of three stages \edit{orchestrated}{enabled} by our novel modules:
First, to capture scene structure and low-frequency appearance, we encode the well-lit input $I_{\rm WL}$ into a latent code $z_{\rm WL} = \mathcal{E}(I_{\rm WL})$. 
%
In parallel, we encode the reference image $I_{\rm LL}$ to obtain a latent code.
%
This code modulates $z_{\rm WL}$ to produce a style-infused latent code $z_0$ following~\citet{chung2024style}. 
%
Second, to transfer high-frequency low-light noise, our Direct-Current-based High-Pass Filter (DHF) module extracts noise components from $I_{\rm LL}$ using Fast Fourier Transform (FFT).
After mean correction, the filtered outputs are encoded by $\mathcal{E}$ to obtain multi-scale high-frequency intermediate features $\{z_1, \dots, z_4\}$ that represent realistic low-light characteristics.
%
Finally, the decoder $\mathcal{D}$ generates the image $\hat{I}_{\rm LL}$ from the latent code $z_0$. During this \edit{synthesis}{process}, our novel Low-light Characteristics Injection Module (LCIM) injects the high-frequency features $\{z_1, \dots, z_4\}$ into the corresponding layers of the decoder. This ensures the faithful rendering of complex noise patterns. 


After we have synthesize low-light image $\hat{I}_{\rm LL}$, we use it for our pose model training.
%
The image is first processed with image backbone and then transformed into a series of tokens $\mathbf{F'}$ by transformer encoder.
%
Following previous work~\cite{edpose}, we initialize human and keypoint queries $\mathbf{Q}$ from $\mathbf{F'}$ and input both into stacks of Deformable Decoder Layers~\cite{deformable-detr}.
%
Within each layer, $\mathbf{Q}$ is first encoded into structured pose prior $\mathbf{Q}_{\rm pose}$ via self-attention.
%
Later, $\mathbf{Q}_{\rm pose}$ query image features $\mathbf{F'}$ via deformable cross attention, producing image cues $\mathbf{Q}_{\rm image}$.
%
We apply Dynamic Control of Attention (DCA) module to adaptively combine $\mathbf{Q}_{\rm pose}$ and $\mathbf{Q}_{\rm image}$, producing new queries $\mathbf{Q}$ for following FFN (feed-forward network) and subsequent layers.
%
At last, each token of $\mathbf{Q}$ is decoded into keypoint coordinates via a simple linear head.
\end{comment}

% \haopeng{In general, overview is a bit too long. We may want to move some details into following sections.}
% \hawk{Rewrote the overview, now just one paragraph. Commented out the old ones, which include three paragraphs. Please check the following section and see if we need to reuse some of the sentences from the old overview.}


% \noindent\textbf{Adaptive Intensity Normalization (AIN)}
% Low-light images often contain extremely low intensity values, which can cause the VAE encoder in the SD model to produce corrupted latent codes.
% %
% To address this, we apply intensity rescaling to both the real low-light reference images and the synthesized low-light outputs generated by our model.
% %
% Specifically, we first scale the input real low-light image $I_\text{LL}$ to a more suitable range using its mean $\mu_{I_\text{LL}}$:
% \begin{equation}
%     I_\text{LL}' = I_\text{LL} \times \frac{\delta}{\mu_{I_\text{LL}}}
% \end{equation}
% where $\delta = 0.449$. 
% %
% After the VAE decoder generates its output $\hat{I}'_\text{LL}$, we rescale this output to match the mean and standard deviation of the original reference low-light image $I_\text{LL}$.
% %
% This standardization and re-scaling process ensures low-light stylistic consistency and is formulated as:
% \begin{equation}
%     \hat{I}_\text{LL} = \frac{\sigma_{I_\text{LL}}}{\sigma_{\hat{I}_\text{LL}'}} (\hat{I}_\text{LL}' - \mu_{\hat{I}_\text{LL}'}) + \mu_{I_\text{LL}}
% \end{equation}
% Here, $\mu$ and $\sigma$ denote the channel-wise mean and standard deviation, respectively. 
% %
% AIN mitigates encoder collapse on low-light inputs and preserves the illumination diversity of the reference images.
%\haopeng{Remove AIN section}


\noindent\textbf{Direct-Current-based High-Pass Filter (DHF)}
% \subsection{Direct-Current-based High-Pass Filter (DHF)}
Our framework extracts high-frequency details by applying a high-pass filter in the frequency domain, yielding an image $I_{\text{HP}}$. It can be formulated as:
\begin{equation}
    I_{\text{HP}} = \text{iFFT}(\text{FFT}(I_\text{LL}) \odot \mathcal{M} )
\end{equation}
%
where $\mathcal{M}$ is a high-pass filter, and $\text{FFT}$ and $\text{iFFT}$ denote the Fast Fourier Transform and its inverse. 
%
By design, $I_{\text{HP}}$ has a mean near zero, with its pixel values representing positive (brighter) and negative (darker) deviations from the local average.
%
A critical challenge arises when preparing $I_{\text{HP}}$ for the SD encoder, which expects inputs normalized to the standard RGB $[0, 1]$ range.
%
Direct clipping of negative values leads to irreversible information loss, especially for darker details, a critical issue in low-light scenarios. 

To address this issue, we introduce a simple yet effective module, DHF.
%
The core idea is to re-center high-frequency details by aligning their distribution with the mean brightness of the original reference image, $I_\text{LL}$.
%
This process preserves the full dynamic range of the extracted details by shifting them into a perceptually meaningful range prior to normalization. 
%
Specifically, we compute the corrected high-frequency image $I_{\text{DHF}}$ as:
\begin{equation}
    I_{\text{DHF}} = I_{\text{HP}} + (\text{mean}(I_\text{LL}) - \text{mean}(I_{\text{HP}})),
\end{equation}
where $\text{mean}(\cdot)$ calculates the global channel-wise mean of an image.
%
This operation ensures that $\text{mean}(I_{\text{DHF}}) = \text{mean}(I_\text{LL})$.
%
By adjusting the negative-valued details, this process reduces information loss during the final clipping to the $[0, 1]$ range. 
%
Consequently, DHF helps preserve both bright and dark high-frequency information, enabling a richer feature representation for low-light domain adaptation.

% \subsection{Low-light Characteristic Injection Module (LCIM)}
\noindent\textbf{Low-light Characteristic Injection Module (LCIM)}
The synthesis process is finally completed in the decoding stage, which generates the low-light image $\hat{I}_{\rm LL}$.
%
A variational autoencoder (VAE) decoder $\mathcal{D}$ takes the style-infused latent code $z_0$, embedding the structure of the well-lit image $I_{\rm WL}$ and the low-frequency style of the reference low-light image $I_{\rm LL}$, and progressively upsamples it.
%
To inject high-frequency details from the reference image into the synthesized low-light output, we introduce LCIM.

After obtaining a set of high-frequency intermediate features, ${z_1,...,z_4}$ from different scales of the high-frequency image $I_\text{DHF}$ produced by DHF, LCIM processes each $z_i$ with a lightweight convolutional layer:
\begin{equation}
    \{f_1, f_2, f_3, f_4\} = \text{LCIM}(\{z_1, z_2, z_3, z_4\}),
\end{equation}

The decoder $\mathcal{D}$ is composed of 4 convolution blocks $d_1,...,d_4$ and a convolution layer $d_\text{final}$. Each processed high-frequency feature ${f_1,...,f_4}$ is injected at the end of each convolution block by adding it to the main stream:
\begin{equation}
    \hat{I}'_\text{LL} \leftarrow d_\text{final}(d_4( d_3( d_2( d_1( z_0 ) + f_1) + f_2) + f_3) + f_4)
\end{equation}

This multi-scale injection strategy guides the synthesis process to render fine-grained low-light noise at appropriate spatial resolutions.
%
Finally, to match the global stylistic appearance of the reference, we align the channel-wise mean and standard deviation of the synthesized image $\hat{I}'_{LL}$ with those of $I_{\rm LL}$ to produce our final output, $\hat{I}_{\rm LL}$.

To optimize LCIM, we freeze the encoder and decoder of the VAE, and train the module to reconstruct low-light images using a composite loss that incorporates both spatial and frequency domains:
\begin{equation}
  \mathcal{L_\mathcal{D}} = \mathcal{L}_{\text{MSE}}(I, \hat{I}) + \lambda \mathcal{L}_{\text{freq}}(I, \hat{I}),
  \label{equ:llcd_loss_revised}
\end{equation}
where $I$ is the low-light input and $\hat{I}$ is its reconstruction. The first term, $\mathcal{L}_{\text{MSE}}$, is the mean squared error, which enforces content fidelity by minimizing pixel-wise differences. The second term, $\mathcal{L}_{\text{freq}}$, is a frequency-domain loss designed to preserve fine-grained details specific to low-light conditions. 
%
The hyperparameter $\lambda$ balances the two loss terms.
%
In particular, the second loss is defined as a weighted MSE on the Fourier magnitude spectra:
\begin{equation}
  \label{eq:freq_loss_revised}
  \mathcal{L}_{\text{freq}} = \frac{1}{MN}\sum_{u=0}^{M-1} \sum_{v=0}^{N-1} \mathcal{W}(u,v) |\mathcal{F}_{I}(u,v) - \mathcal{F}_{\hat{I}}(u,v)|^{2},
\end{equation}
where $\mathcal{F}_{I}$ and $\mathcal{F}_{\hat{I}}$ are the Fourier magnitude spectra of the input and reconstructed images, respectively, and $(M,N)$ is the image resolution. The weighting function $\mathcal{W}(u,v)$ is defined as:
\begin{equation}
  \label{eq:weighting_revised}
  \mathcal{W}(u,v) = \sin{\left(\frac{\pi|2u-M|}{2M}\right)} + \sin{\left(\frac{\pi|2v-N|}{2N}\right)}.
\end{equation}
This sinusoidal weighting scheme prioritizes mid-to-high frequency components, aiming to enhance perceptual quality and retain low-light characteristics without introducing over-sharpening artifacts. 
%
Although LCIM is trained with a reconstruction objective, it operates on high-frequency components extracted from low-light images, which mainly capture noise patterns. Thus, LCIM captures transferable low-light characteristics that can be applied to synthesize low-light effects for different input images.


% \subsection{Dynamic Control of Attention (DCA)}
\noindent\textbf{Dynamic Control of Attention (DCA)}
%
\input{figures/l2norm_compare}
%
After synthesizing the low-light image $\hat{I}_\text{LL}$, we use it for our pose model training.
%
$\hat{I}_\text{LL}$ is first processed with a feature extractor and then transformed into tokens $\mathbf{F'}$ by a Transformer encoder.
%
We denote the visual tokens carrying image cues after deformable cross-attention as $\mathbf{Q}_\text{image}$ (corresponding to the output of deformable token-to-human/keypoint attention in \cite{edpose}).
%
Our pose model also initializes keypoint latents and performs self-attention among them, forming a pose-prior representation denoted as $\mathbf{Q}_\text{pose}$ (corresponding to the output of human-to-keypoint interactive attention in \cite{edpose}).
%
Within each deformable decoder layer, we need to fuse the pose prior latent $\mathbf{Q}_\text{pose}$ from self-attention and image cues latent $\mathbf{Q}_\text{image}$ from deformable cross-attention.
%
Existing DETR-based human pose estimators~\cite{edpose,grouppose,tan2024diffusionregpose} (built on~\cite{DETR,deformable-detr}) directly sum $\mathbf{Q}_\text{pose}$ and $\mathbf{Q}_\text{image}$ before the feedforward network (FFN), a rigid design that leads to degraded performance under low-light conditions.


Following the analysis framework of~\citet{elhage2021mathematical,kim2025peri}, we evaluate the ratio of Frobenius Norm of $\mathbf{Q}_\text{image}$ and $\mathbf{Q}_\text{pose}$ in typical low-light conditions that one or more human joints are barely visible under low-light conditions, as shown in~\cref{fig:l2norm-vis}.
%
When both knees are nearly indistinguishable from the background, the ratio remains approximately $1.7$, comparable to that of the clearly visible keypoints.
%
In fact, across a set of well-lit images, this ratio remains stable with a mean around $1.68$.
%
This clearly demonstrates that rigid summation fails to reduce the contribution of unreliable image cues when keypoints are barely visible, leading to incorrect pose estimation for both knees as shown in~\cref{fig:l2norm-before}.


To address this issue, we introduce DCA, which adaptively fuses the pose prior latent $\mathbf{Q}_\text{pose}$ from self-attention and image cues latent $\mathbf{Q}_\text{image}$ from deformable cross-attention.
%
DCA first concatenates $\mathbf{Q}_\text{pose}$ and $\mathbf{Q}_\text{image}$ in channel dimension as $\mathbf{Q}_\text{cat}$,
\begin{equation}
\mathbf{Q}_\text{cat} = \text{Concat}(\mathbf{Q}_\text{pose}, \mathbf{Q}_\text{image}).
\end{equation}
%
Then, $\mathbf{Q}_\text{cat}$ is fed into a two-layer MLP that reduces the channel dimension to two.
%
A softmax function is then applied to produce two competitive weights corresponding to the pose-prior and image-cue features,
\begin{equation}
(\mathbf{w}_\text{pose}, \mathbf{w}_\text{image}) = \text{softmax}(\text{MLP} (\mathbf{Q}_\text{cat})).
\end{equation}
%
where $\mathbf{w}_\text{pose}$ and $\mathbf{w}_\text{image}$ are the obtained weights for $\mathbf{Q}_\text{pose}$ and $\mathbf{Q}_\text{image}$.
We then apply Hadamard product of the weights and their corresponding latent, where the new queries $\mathbf{Q}$ for the subsequent FFN and following layers are obtained by a weighted sum of $\mathbf{Q}_\text{pose}$ and $\mathbf{Q}_\text{image}$,
\begin{equation}
\mathbf{Q} = \mathbf{w}_\text{pose} \odot \mathbf{Q}_\text{pose} \oplus \mathbf{w}_\text{image} \odot \mathbf{Q}_\text{image}.
\end{equation}
%
Notably, DCA assigns different weights for different keypoints of a human instance, allowing the model to rely more on pose priors when a keypoint is less visible, and more on image cues when a keypoint is visible.
%
With only two additional linear layers, DCA enables the model to balance the influence of image cues and pose prior, leading to improved performance under low-light conditions as shown in~\cref{fig:l2norm-vis,fig:l2norm-after}.


\noindent\textbf{Pose Estimation Training}
% \subsection{Pose Estimation Training}
%
For the human pose estimation model, we adopt the loss formulation from ED-Pose~\cite{edpose}. We employ a set-based Hungarian loss that forces
a unique prediction for each ground-truth box and keypoint. The total loss is a weighted sum of classification $\mathcal{L}_c$, human box regression $\mathcal{L}_h$, and keypoint regression loss $\mathcal{L}_k$. Notably, $\mathcal{L}_k$ simply
consists of the normal L1 loss and the constrained L1 loss named Object Keypoint Similarity (OKS) loss~\cite{rw-petr} without any dense supervision (e.g., heatmap). Please refer to the supplementary material for details.

% \begin{equation}
%   \mathcal{L}_{\text{pose}} = \mathcal{L}_{\text{heatmap}} + \gamma \mathcal{L}_{\text{offset}}.
% \end{equation}




\section{Experiment}
\label{sec:exp}
%
% \subsection{Implementations and dataset}
% We provide more details in supplementary.


\noindent\textbf{Datasets}
We evaluate UDAPose on the ExLPose dataset~\cite{ExLPose_2023_CVPR}, specifically designed for benchmarking 2D human pose estimation in extremely low-light conditions.
%
% \edit{The ExLPose training set consists of 2,065 well-lit and optically filtered low-light image pairs, with pose annotations following the CrowdPose format.
% %
% These images span 251 indoor and outdoor scenes, with low-light versions generated using a dual-camera system under varying conditions to simulate diverse low-light scenarios. }{}
ExLPose provides two distinct test sets: ExLPose-OCN and ExLPose-test.
%
ExLPose-OCN contains 360 real low-light images captured at night using A7M3 and RICOH3 cameras.
%
ExLPose-test consists of 491 optically filtered images, where brightness is reduced by a factor of 100.
%
ExLPose-test, also referred to as Low-Light All (LL-A), is further divided into three difficulty levels: Low-Light Normal (LL-N), Low-Light Hard (LL-H), and Low-Light Extreme (LL-E).


To validate our method's generalization ability, we performed cross-dataset evaluation on EHPT-XC~\cite{ehpt-xc}.
%
EHPT-XC is a novel hybrid dataset combining RGB and event data, specifically designed for human pose estimation and tracking in challenging low-light and motion blur conditions.
%
% \edit{
% It encompasses RGB video frames from 158 diverse sequences, along with pixel-wise aligned and temporally synchronized event streams, and annotations containing 38K 2D keypoints and bounding boxes with track IDs.}{}
%
Given that some RGB data in EHPT-XC primarily exhibits motion blur without low-light conditions, we combined the train and test split of EHPT-XC and selected a specific subset of 12 scenes (1200 images) under low-light conditions for cross-dataset evaluation.
%
% \edit{This subset allows us to assess method performance under unseen low-light scenarios.}{}

\input{tables/tab_exlpose-test-AP}


\noindent\textbf{Evaluation metrics}
%
% Our evaluation follows the COCO protocol~\cite{dataset-coco}, as used in LSBN+LUPI~\cite{ExLPose_2023_CVPR}, for testing on both the ExLPose-test and ExLPose-OCN datasets.
We evaluate our method following the COCO evaluation protocol~\cite{lin2014microsoft}, consistent with exisiting methods~\cite{ExLPose_2023_CVPR,ella-eccv, ehpt-xc}, on ExLPose-test, ExLPose-OCN, and EHPT-XC.
%
% For each subset, we report Average Precision across multiple thresholds (i.e., AP@0.5:0.95) as the performance metric.
For each subset, we report Average Precision (AP) and Average Recall (AR) across multiple thresholds (@0.5:0.95) as the primary performance metrics.


\noindent\textbf{Implementation details}
%
We adopt SD-2.1-base as our backbone model for low-light data synthesis.
%
During training data synthesis, we use DDIM~\cite{song2020ddim} as our solver and 50 steps in sampling process.
%
% \edit{For training LICM, we combine ExLPose-test low-light images and ExLPose-OCN images as our unlabeled low-light dataset while keeping the encoder parameters frozen. Our training process involves randomly cropping images to $512 \times 512$ pixels and applying random flipping for data augmentation.}{}
%
We train LCIM using Adam optimizer~\cite{kingma2014adam} over 400
epochs in total, with an initial learning rate of $4 \times 10^{-6}$ that decreases
to $4 \times 10^{-7}$ after 300 epochs.
%
We train with a batch size of 32 across 4 NVIDIA RTX4090 GPUs and set the
weight $\lambda$ in~\cref{equ:llcd_loss_revised} to $4 \times 10^{-4}$ during training
%
% Our framework uses DEKR-W32~\cite{DEKR2021} as the backbone for the human pose estimation model to ensure a fair comparison with the recent low-light human pose estimation approach ELLA~\cite{ella-eccv}.
%
Our framework uses ED-Pose~\cite{edpose} with Swin-T~\cite{liu2021swin} pretrained on ImageNet 22k~\cite{deng2009imagenet} as the backbone for the human pose estimation model.
%
Training is performed with a batch size of 16 on 2 NVIDIA RTX PRO 6000 Blackwell GPUs.
%
% \edit{During training, we resize input images to $512 \times 512$ and apply data augmentations following DEKR, including random rotation ($\pm30^\circ$), scaling (0.75–1.5×), translation ($\pm40$ pixels), and flipping. We adopt the same training strategy as DEKR, with the only modification being the loss weighting factor $\gamma = 0.03$.}{}

% \noindent
% \textbf{Baselines } For comparative evaluation, we benchmark against state-of-the-art
% and highly cited methods in two categories: image enhancement (RFormer, LLFlow
% and QuadPrior~\cite{cai2023retinexformer,LLFlow,quadprior}) and domain adaptation
% (UDA-HE, AdvEnt, CycleGAN, UNIT, UNSB~\cite{CycleGAN2017,UNIT,kim2023unsb,AdvEnt,kim2022unified}).
% We also include ELLA~\cite{ella-eccv}, the current SOTA method for low-light human
% pose estimation, in our comparison.
% %
% To establish a fair comparison framework, we utilize the same base human pose
% estimator, DEKR~\cite{DEKR2021}, across all methods including our own.
% %
% Following ExLPose's~\cite{ExLPose_2023_CVPR} methodology, we modified AdvEnt~\cite{AdvEnt}
% by replacing its semantic segmentation backbone with our 2D pose estimator.
% %
% For UDA-HE~\cite{kim2022unified}, which originally operates as a model-agnostic
% domain-adaptive human pose estimation method, we upgraded its ResNet backbone to
% HRNet (matching our method's backbone) and retrained the AdaIN component to ensure
% equitable comparison.
% %
% It's worth noting that UDA-HE employs a bottom-up paradigm.
% %
% We also compare our framework to ELLA~\cite{ella-eccv}, the SOTA method of low-light
% human pose estimation.
% %
% Note that we have the same pose model settings as the main teacher and student in
% ELLA~\cite{ella-eccv}. However, the student model in ELLA distillates from dual teachers.
% %
% As our work main focus on data synthesis, we do not conflict with the teacher-student
% framework.
% %
% For fairness, our pose model training is well-aligned with the main teacher training
% and compare to it.
% %
% We discuss the the comparison to the full model proposed in ELLA~\cite{ella-eccv}
% in Supplementary.


% For domain-adaptive baselines, we modify AdvEnt~\cite{AdvEnt} following ExLPose~\cite{ExLPose_2023_CVPR} by replacing its semantic segmentation backbone with our 2D pose estimator. Similarly, UDA-HE~\cite{kim2022unified}, originally designed as a model-agnostic approach, is adapted by upgrading its ResNet backbone to HRNet (matching our model) and retraining its AdaIN module to ensure consistency. 

\noindent\textbf{Baselines} For comparative evaluation, we benchmark against state-of-the-art methods in two categories: image enhancement (RFormer, DarkIR, QuadPrior, and LightenDiff~\citep{cai2023retinexformer,feijoo2025darkir,quadprior,jiang2024lightendiffusion}) and domain adaptation (CycleGAN, UNIT, UDA-HE, UNSB, EnCo~\citep{CycleGAN2017,UNIT,kim2022unified,kim2023unsb,cai2024enco}).
%
We also include ELLA~\cite{ella-eccv}, the state-of-the-art (SOTA) method for low-light human pose estimation.
%
To ensure a fair comparison, we use ED-Pose~\cite{edpose} as the backbone network across all methods, including our own.
%
While ELLA~\cite{ella-eccv} adopts a dual-teacher-student framework, where the student model distillates from dual teachers utilizing low-light images, our method instead focuses on low-light synthesis and balancing pose priors and visual cues.
% {This sentence is wrong? Using low-light training images?}
% \haopeng{Not precise enough. In knowledge acquisition stage, student would utilize degraded real LL (from ExLPose LL dataset) with pseudo labels from teachers for training.} 
%
To evaluate the performance of data synthesis, the low-light data augmentation part of ELLA is applied in the comparison.
%
A full comparison to ELLA’s complete dual-teacher-student framework is provided in the supplementary material.
%
% \edit{To show the effectiveness and necessity of our method, we also include zero-shot performance from Sapiens. Note that as Sapiens is a top-down method, we directly use the ground-truth bounding box to crop out single human instance as input, leading to extra advantages compared to other baselines and our pose model. As QuadPrior is a source-free method, we directly use authors' provided checkpoint trained on COCO to have best performance. Also, LightenDiff requires pair images in different illumination level to train, which is not feasible in ExLPose dataset. We also use authors' provided checkpoint to have best performance.}{}


\subsection{Performance on ExLPose-test}
%
%
\input{tables/tab_exlpose-test-AR}
%
As shown in~\cref{tab:exlpose-test-AP,tab:exlpose-test-AR}, UDAPose consistently outperforms all baselines on the ExLPose-test set. On average across all low-light conditions (LL-A), UDAPose achieves 27.0 AP and 36.5 AR, surpassing the strongest baseline, CycleGAN~\cite{CycleGAN2017} and ELLA~\cite{ella-eccv}, by 7.4 AP (a 37.8\% relative improvement) and 7.6 AR (a 26.3\% relative improvement), respectively. 
%
The performance gap widens as lighting conditions deteriorate. Specifically, UDAPose leads by 5.0 AP and 2.6 AR on the normal subset (LL-N) and by 10.1 AP (a 56.4\% relative gain) and 9.4 AR (a 33.6\% relative gain) on the hard subset (LL-H).
%
The advantage is clearest on the extreme subset (LL-E), where UDAPose delivers a more than three-fold improvement over ELLA on AP (11.7 vs. 3.4 AP) and more than double on AR (20.4 vs. 9.7 AR). Our method outperforms all baselines across diverse low-light conditions.


\subsubsection{Qualitative Analysis}
%
\input{figures/representative_result}
%
\cref{fig:qualitative} provides a qualitative comparison against representative methods. In normal low-light conditions, UDAPose already yields more precise joint localization. As lighting degrades, our superiority becomes more evident. 
%
In hard low-light, competing methods produce poses with significant limb errors, whereas UDAPose maintains an accurate skeletal structure. Under extreme low-light, where the subject is barely visible, other methods generate fragmented and anatomically implausible poses. In contrast, UDAPose successfully reconstructs a complete and coherent human pose. These visual results support our quantitative findings, confirming that our synthetic data generation and adaptive fusion of learned pose priors and image cues enable robust pose estimation in challenging low-light scenarios.




\subsection{Performance on ExLPose-OCN}
\input{tables/tab_exlpose-ocn}
%
\cref{tab:exlpose-ocn} presents our quantitative results on the ExLPose-OCN dataset. Our model achieves an average AP of 51.4 and an average AR of 65.1, a 5.4 AP improvement (11.7\% relative gain) and a 2.8 AR improvement (4.5\% relative gain) over the previous state-of-the-art~\cite{ella-eccv}. 
% %
% While our method surpasses most baselines, Sapiens~\cite{khirodkar2024sapiens} also performs well. 
% %
% We attribute this to the nature of the OCN dataset, which often contains localized light sources that illuminate some joints while obscuring others. 
% %
% Sapiens' extensive pre-training and ability to handle occlusions make it well-suited for these partially visible scenarios.
% To further explore the impact of a strong well-lit pose foundation, we introduce a variant, ``Ours (CrowdPose)''. This model is first pre-trained on the large-scale CrowdPose dataset~\cite{li2019crowdpose} and then adapted using our synthetic low-light data. 
% %
% This pre-training strategy alone improves performance by about 12 AP, resulting in a final average AP of 48.4. 
% %
% Crucially, this enhanced model significantly outperforms Sapiens by 7.8 AP and 8.8 AP on the A7M3 and RICOH3 subsets, respectively. 
% %
% This is especially notable given that Sapiens is trained on a much larger dataset and requires ground-truth bounding boxes, an advantage our bottom-up method does not have.  
%
These results show that our approach enables robust pose estimation in real-world low-light conditions where annotated data is scarce.

\input{tables/tab_zero-shot}

\input{tables/tab_abl}

\subsection{Cross-dataset validation on EHPT-XC}
%
To assess our model's generalization ability, we perform a cross-dataset validation on the EHPT-XC dataset~\cite{ehpt-xc}, which features challenging real-world conditions such as motion blur and low light.
%
As shown in~\cref{tab:zero-shot}, our method consistently outperforms all state-of-the-art baselines across all Average Precision (AP) and Average Recall (AR) metrics.
%
Specifically, our approach achieves an AP@0.5:0.95 of 31.0, surpassing the strongest baseline, ELLA~\cite{ella-eccv}, by 7.4 points.
%
This strong performance also extends to other metrics, highlighting our model’s ability to generalize to unseen and degraded data without fine-tuning.


% \subsubsection{Analysis of Key Components}
% As shown in Table~\ref{tab:abl}, we incrementally add our proposed modules to a baseline model to demonstrate their effectiveness.


\subsection{Ablation Studies}




\subsubsection{Baselines}
We first establish two baselines. A standard pose estimator trained only on well-lit data fails on low-light images (e.g., 3.4 AP on LL-N), highlighting a significant domain gap. 
Adapting this model with a simple histogram matching technique offers only a marginal improvement (21.3 AP on LL-N), indicating that basic color transformations are insufficient. 
A second baseline, ``Baseline SD'', following~\citet{chung2024style}, achieves descent performance by synthesizing low-light images (23.7 AP on LL-N) but still struggles with more challenging conditions (7.2 AP on LL-H).

\subsubsection{Component Analysis}
As shown in~\cref{tab:abl}, building on ``Baseline SD'', we first integrate LCIM, which yields the most substantial performance leap. The LCIM dramatically improves results on the most difficult subsets, increasing the AP on LL-H from 7.2 to 20.7 and on LL-E from 0.0 to 7.8.
%
This highlights the importance of LCIM in transferring low-light features from the reference image.
%
In addition, the DHF module improves performance by modeling frequency-domain attributes, delivering notable performance gains on challenging data (LL-H: +4.6 AP, LL-E: +1.6 AP).
%
Lastly, DCA is added to improve our pose model's capability to deal with low-visibility conditions, leading to consistent improvement across all subsets, from LL-N (+3.4 AP) to more challenging LL-H (+2.7 AP) and LL-E (+2.3 AP).
% \subsubsection{Full Model}
% Finally, our ``Pair-guided'' training strategy further optimizes the framework. 
% %
% While it involves a minor performance trade-off on some subsets (e.g., -0.8 AP on LL-H), it improves performance on well-lit data (+1.2 AP on WL) and achieves the best overall results.
% More importantly, this strategy streamlines the training process into a single, efficient stage. 
% %
Overall, each component plays a clear role, and together they improve the model’s ability to handle varied low-light scenarios.

\input{tables/tab_abl-skip}

\subsubsection{Analysis of LCIM}
\label{sec:ablation_skips}
We now analyze the core of our LCIM module: the multi-scale intermediate features. As detailed in~\cref{tab:abl-skip}, we start with a baseline model ($z_0$) that omits all intermediate features, then progressively integrate features from coarse to fine levels ($z_1$ to $z_4$). 
The $z_0$ model, achieves a modest 40.0 AP on A7M3 and 36.8 AP on RICOH3.

These results show that fusing multi-scale features is important. 
%
Each added intermediate feature brings a consistent performance improvement. 
%
Adding all four feature levels ($+z_1+z_2+z_3+z_4$) results in our strongest model, improving the AP by +15.0 on A7M3 (40.0$\rightarrow$55.0) and +11.1 on RICOH3 (36.8$\rightarrow$47.9) compared to the $z_0$ baseline. 
%
This analysis shows that our coarse-to-fine fusion strategy effectively uses multi-scale latent features from the SD encoder, which is important for robust pose estimation under challenging low-light conditions.




% \subsection{Anatomical Consistency}
% \haopeng{Consider move to supp.}
% %
% \input{tables/tab_consistency}
% %
% We evaluate the anatomical consistency of our generated low-light images, a critical factor for reusing pose annotations from well-lit images.
% %
% To this end, we synthesize low-light images from the ExLPose dataset and compare them against ground-truth images using a comprehensive set of metrics.
% %
% We assess image fidelity at the pixel level with PSNR and SSIM, and at the feature level with LPIPS and Fr\'echet Inception Distance (FID).
% %
% More importantly, to directly quantify anatomical integrity, we compute the Kullback–Leibler (KL) divergence between pose keypoint heatmaps. These heatmaps are inferred by a pre-trained pose estimator from our synthetic images versus the ground-truth images.

% As presented in Table~\ref{tab:consistency}, our method significantly outperforms all baselines across every metric.
% %
% It achieves a PSNR of 41.13 and an SSIM of 0.91, indicating superior pixel-level accuracy.
% %
% Furthermore, our method obtains the lowest LPIPS (0.20) and a remarkably low FID of 11.17, confirming that the generated images have higher perceptual quality and a feature distribution much closer to that of real images.
% %
% Crucially, our method yields a KL divergence of only 0.008, which is an order of magnitude lower than the best-performing baseline (CycleGAN: 0.028). This result provides direct evidence that our generation process preserves the underlying human anatomical structure with high precision.
% %
% Consequently, the pose information extracted from our synthetic data is nearly identical to that from real low-light images, validating our method's effectiveness for downstream pose estimation tasks.





% \subsection{Qualitative results}
% \haopeng{Move to supp.}
% qualitative comparison
% \input{figures/qualitative}
%
% We present a qualitative comparison between our UDAPose framework and existing methods in \cref{fig:gen-result-comp}. 
% %
% The visual results clearly demonstrate the superior capability of our approach in generating realistic low-light images that closely resemble the real low-light ground truth.

% Examining the enhancement-based method, QuadPrior~\cite{quadprior} attempts to brighten low-light images but tends to produce over-smoothed results with significant loss of texture and detail.
% %
% Among image-to-image translation methods, CycleGAN~\cite{CycleGAN2017} produces images with excessive color shifts and unrealistic noise patterns. 
% %
% UNIT~\cite{UNIT} and UNSB~\cite{kim2023unsb} generate images with irregular noise distributions that significantly differ from real low-light conditions, making them less effective for training robust pose estimation models. 
% %
% StyleID~\cite{chung2024style}, while better at preserving the overall scene structure, still struggles to accurately capture the complex noise patterns characteristic of low-light photography.

% In contrast, our UDAPose framework generates low-light images that exhibit remarkably realistic noise characteristics. 
% %
% The synthetic images produced by our method faithfully preserve essential high-frequency details while accurately modeling the complex noise patterns present in real low-light conditions. 
% %
% The superior quality of our synthetic low-light images can be attributed to the CIM module, which effectively captures and transfers the complex low-light characteristics from unpaired real low-light images to well-lit inputs. 
% %
% By leveraging Stable Diffusion's generative capabilities combined with our CIM, UDAPose overcomes the limitations of previous approaches, generating more realistic training data that better prepares the pose estimation model for real-world low-light scenarios.
% We present a qualitative comparison of UDAPose against existing methods in Figure~\ref{fig:gen-result-comp}, demonstrating its superior ability to generate realistic low-light images that closely resemble real low-light ground truth.

% For enhancement-based methods, QuadPrior~\cite{quadprior} brightens low-light images but produces over-smoothed results, leading to a loss of texture and fine details. Among image-to-image translation approaches, CycleGAN~\cite{CycleGAN2017} introduces excessive color shifts and unrealistic noise patterns, while UNIT~\cite{UNIT} and UNSB~\cite{kim2023unsb} generate irregular noise distributions that fail to match real low-light characteristics, making them less effective for training pose estimation models. StyleID~\cite{chung2024style} better preserves scene structure but still struggles to capture the complex noise patterns inherent to low-light conditions.

% In contrast, UDAPose generates synthetic low-light images that exhibit realistic noise characteristics and faithfully preserve essential high-frequency details. The improvements stem from our LCIM module, which effectively captures and transfers complex low-light characteristics from unpaired real low-light images to well-lit inputs. By integrating Stable Diffusion’s generative capabilities with LCIM, UDAPose overcomes the limitations of prior methods, producing high-quality synthetic training data that significantly enhances pose estimation in real-world low-light scenarios. We provide more qualitative results and further discussion in the supplementary material.




\section{Conclusion}
\label{sec:con}
%
In this work, we introduced UDAPose, a novel domain-adaptive framework for human pose estimation under low-light conditions.
%
UDAPose leverages SD to synthesize low-light images, incorporating the DHF with LCIM to retain key low-light details.
%
UDAPose also integrates DCA to balance unreliable visual cues under poor illuminated conditions with learned pose priors. 
%
This results in improved performance under extreme lighting conditions.
%
Our approach outperforms both rule-based and learning-based augmentation methods, achieving substantial performance gains on ExLPose and EHPT-XC.
%
These results demonstrate UDAPose’s effectiveness in addressing limitations of existing low-light human pose estimation methods and improving human pose estimation performance in real-world low-visibility scenarios.



==> sec/main_paper.tex <==
\begin{abstract}
%
Low-visibility scenarios, such as low-light conditions, pose significant challenges to human pose estimation due to the scarcity of annotated low-light datasets and the loss of visual information under poor illumination. 
%
Recent domain adaptation techniques attempt to utilize well-lit labels by augmenting well-lit images to mimic low-light conditions.
%
But handcrafted augmentations oversimplify noise patterns, while learning-based methods often fail to preserve high-frequency low-light characteristics, producing unrealistic images that lead pose models to generalize poorly to real low-light scenes.
%
Moreover, recent pose estimators rely on image cues through image-to-keypoint cross-attention, but these cues become unreliable under low-light conditions.
%
To address these issues, we propose Unsupervised Domain Adaptation for Pose Estimation (UDAPose), a novel framework that synthesizes \edit{realistic}{} low-light images and dynamically fuses visual cues with pose priors for improved pose estimation.
%
Specifically, our synthesis method incorporates a Direct-Current-based High-Pass Filter (DHF) and a Low-light Characteristics Injection Module (LCIM) to inject high-frequency details from input low-light images, overcoming rigidity or the detail loss in existing approaches.
%
Furthermore, we introduce a Dynamic Control of Attention (DCA) module that adaptively balances image cues with learned pose priors in the Transformer architecture.
%
Experiments show that UDAPose outperforms state-of-the-art methods, with notable AP gains of 10.1 (56.4\%) on the challenging ExLPose-test hard set (LL-H) and 7.4 (31.4\%) in cross-dataset validation on EHPT-XC.
%
Code is available at \href{https://github.com/Vision-and-Multimodal-Intelligence-Lab/UDAPose}{VMIL/UDAPose}.
\end{abstract}



\section{Introduction}
\label{sec:intro}
%
\input{figures/fig_baseline_comp}
%
Human pose estimation is a foundational task in computer
vision, essential for many downstream applications~\cite{application-healthcare,application-traffic,application-sports2,application-ar,application-security,survey-application-2021}.
%
Existing methods~\cite{rw-poseur,purkrabek2025probpose,rw-swahr,LOGOCAP,grouppose,tan2024diffusionregpose}
and benchmark datasets~\cite{lin2014microsoft,li2019crowdpose,dataset-ochuman}
primarily focus on well-illuminated scenarios.
%
However, real-world scenarios often involve low-light conditions, which significantly degrade pose estimation performance~\cite{ExLPose_2023_CVPR,ehpt-xc} and result in safety risks~\cite{tesla-NHTSA}. 
%
A key challenge is the scarcity of real-world low-visibility datasets, as annotating such images is inherently difficult.
%
\citet{ExLPose_2023_CVPR} introduced a specialized camera system to capture paired well-lit and low-light images, transferring annotations from well-lit to low-light counterparts.
%
However, these artificially darkened images cannot fully replicate real
low-light conditions, limiting the generalization of models trained on them~\cite{li2021learning}.
%
Although event cameras~\cite{ehpt-xc} offer an alternative, they require specialized hardware and complex cross-modality alignment, which limits scalable deployment.


While paired data collection is impractical, an alternative approach is to apply low-light image enhancement methods~\cite{yang2023implicit,quadprior,cai2023retinexformer,feijoo2025darkir,jiang2024lightendiffusion}.
%
However, this recovery process is inherently ill-posed, as reconstructing missing visual details from severely degraded images is challenging and often leads to artifacts that negatively impact human pose estimation.\textbf{}
%
Instead of recovering lost details, domain-adaptive methods~\cite{ella-eccv,kim2022unified} take a different approach by synthesizing low-light images from well-lit ones to mimic low-visibility conditions.
%
This allows models to leverage existing well-lit annotations during training.
%
These methods typically rely on handcrafted augmentations~\cite{ella-eccv} or learning-based image-to-image translation~\cite{CycleGAN2017,cai2024enco,kim2023unsb} to bridge the domain gap.
%
However, their effectiveness depends on how well they replicate real low-light characteristics, which remains a significant and underexplored challenge.


Handcrafted augmentations often fail to replicate the complex characteristics of real low-light images.
%
For instance, ELLA~\cite{ella-eccv} applies Gaussian white noise to simulate low-light conditions. 
%
However, real low-light noise, such as photon noise, thermal noise, and quantization noise, is far more complex~\cite{wei2021physics}. 
%
% \edit{Moreover, rule-based augmentations lack flexibility, as they are designed for specific low-light conditions.}
Moreover, handcrafted augmentations exhibit limited flexibility and generalization, as they are tailored to specific low-light scenarios. 
%
Consequently, their deployment in novel environments, such as those involving different camera hardware or new datasets (e.g., EHPT-XC~\citep{ehpt-xc}), often results in suboptimal performance and requires extensive manual tuning.
%
Learning-based augmentations utilize unpaired image-to-image translation~\cite{CycleGAN2017, kim2023unsb, chung2024style} to adapt well-lit images to low-light conditions.
%
However, as shown in~\cref{fig:intro-baseline-gen-comp}, these methods fail to replicate realistic low-light characteristics. 
%
CycleGAN~\cite{CycleGAN2017} tends to overly darken images while introducing lighting artifacts, while StyleID~\cite{chung2024style} fails to generate realistic low-light noise.


Beyond the limitations of low-light data synthesis, the robustness of modern pose estimators themselves becomes a critical factor, particularly the recent one-stage architectures~\cite{edpose,grouppose,tan2024diffusionregpose}.
%
When visual cues are subtle or entirely absent, a robust model should leverage learned pose priors to infer keypoints hidden in darkness.
%
However, recent one-stage pose estimators~\cite{edpose,grouppose,tan2024diffusionregpose}, often built upon DETR-like architectures~\cite{DETR,deformable-detr}, utilize cross-attention to query image features and fuse them with pose priors via a direct residual connection. 
%
This rigid summation biases the fused representation toward image cues, even when the visual information is unreliable, particularly under low-light conditions.
%
Empirically, we observe that the model consistently emphasizes cross-attention visual features over pose-prior features under both well-lit and low-light conditions (see~\cref{fig:l2norm} for L2-norm comparisons).
%
Consequently, under poor illumination, noisy and unreliable visual features still contribute significantly compared to the pose priors, leading to unreliable human pose predictions, particularly for the low-visibility keypoints.
% \yihao{This sentence suggests that the previous method already considers pose priors, but it is not clear why this leads the model to heavily rely on image cues. Even though the next sentence attributes this to the rigid summation of image and prior features, the explanation is still not explicit. Perhaps we can soften the tone and clarify the mechanism, e.g., “we found that with rigid summation, the model tends to emphasize image cues regardless of their visibility.” After that, we could reference the quantitative results (L2-norm/eigen value)or visual examples to support this point."}


To overcome the above limitations, we propose UDAPose, a novel framework for unsupervised domain adaptation in human pose estimation.
%
Our framework employs Stable Diffusion (SD)~\cite{latentdiffusion} as a generative backbone to synthesize \edit{realistic}{} low-light images from well-lit ones.
%
By using unlabeled low-light images as references, UDAPose synthesizes augmentations that better reflect real low-light characteristics, outperforming existing approaches.
%
Our approach is highly practical, as collecting unlabeled low-light images is far easier than obtaining corresponding pose annotations.
%
\edit{To further enhance realism}{To capture low-light characteristics from reference images}, we introduce (1) Direct-Current-based High-Pass Filter (DHF), which extracts high-frequency low-light characteristics and (2) Low-Light Characteristics Injection Module (LCIM), which ensures that synthesized images retain complex low-light features of the reference images.
%
Unlike existing learning-based augmentations, UDAPose preserves essential low-light characteristics for human pose estimation, achieving significant performance gains.
%
A representative example is shown in the last column of~\cref{fig:intro-baseline-gen-comp}.


To address the vulnerability of pose estimation models under low-light conditions, we introduce the Dynamic Control of Attention (DCA) module. 
%
DCA adaptively controls the fusion weight between visual cues and pose priors, allowing the model to dynamically adjust the contributions from image features and learned human pose priors when visual information is degraded.
%
In summary, our contributions are as follows. 
\begin{itemize}
    \item 
    We propose UDAPose, an unsupervised domain adaptation framework that augments well-lit images to mimic low-light conditions and adaptively fuses visual cues with learned pose priors, achieving improved low-light human pose estimation without requiring low-light annotations.
    \item 
    We introduce the Direct-Current-based High-Pass-Filter (DHF) and Low-Light Characteristics Injection Module (LCIM), which preserve and inject \edit{realistic}{} high-frequency details to the synthesized low-light images.
    \item
    We propose Dynamic Control of Attention (DCA), which dynamically balances image cues with learned pose priors in the Transformer architecture, reducing the influence of noisy and unreliable visual cues in low-light scenarios. 
\end{itemize}
%
Experimental results show UDAPose surpasses existing methods, achieving a 10.1 AP (56.4\%) improvement on the low-light hard set (LL-H) of ExLPose-test and a 7.4 AP (31.4\%) improvement in cross-dataset evaluation on EHPT-XC, highlighting its robustness under low-light conditions.




\section{Related Work}
\label{sec:related}
%
\noindent\textbf{Human Pose Estimation}
Modern human pose estimation is primarily categorized into two mainstream paradigms: top-down and bottom-up. Top-down approaches~\cite{rw-poseur,wang2024locllm,purkrabek2025probpose} first detect individuals and subsequently estimate the pose for each one. In contrast, bottom-up approaches~\cite{DEKR2021,rw-swahr,LOGOCAP} first detect all body keypoints in the image and then assemble them into distinct person instances.
%
Recent advances, including one-stage unified detection-estimation frameworks~\cite{tian2019directpose,mao2021fcpose,shi2021inspose,xiao2022querypose,edpose,grouppose,tan2024diffusionregpose} and Vision Transformer-based models~\cite{rw-petr,xu2022vitpose,wang2024locllm,khirodkar2024sapiens}, have achieved remarkable accuracy. 
%
However, these models are trained and evaluated primarily on benchmarks with ideal lighting conditions~\cite{lin2014microsoft,li2019crowdpose,dataset-lsp,dataset-ochuman}. In particular, recent one-stage methods~\cite{edpose,grouppose,tan2024diffusionregpose} that rely on image cues become unreliable under low-light conditions.
%
Consequently, their performance degrades significantly in low-light scenarios~\cite{ExLPose_2023_CVPR,ehpt-xc}. 
%
While some works have explored domain adaptation~\cite{kim2022unified, peng2023source, raychaudhuri2023prior, cao2019cross, li2021synthetic, mu2020learning, han2022learning, jiang2021regressive, jin2022multibranch} or simple rule-based augmentations~\cite{ella-eccv}, they either lack specific designs for low-light characteristics or fail to synthesize realistic degradation. 
%
Methods requiring paired low-light and well-lit images~\cite{ExLPose_2023_CVPR}, or additional event camera data~\cite{ehpt-xc} are impractical due to the difficulty of collecting such data at scale and their limited scalability in deployment.

\noindent\textbf{Low-light Image Enhancement}
An intuitive approach for low-light pose estimation is to first apply a low-light image enhancement (LLIE) method as a pre-processing step. 
%
While deep learning techniques, including CNNs~\cite{moran2020deeplpf, sharma2021nighttime, wang2019underexposed}, GANs~\cite{huang2017arbitrary, jin2022unsupervised, jiang2021enlightengan, yang2023implicit}, Transformers~\cite{cai2023retinexformer,feijoo2025darkir}, and diffusion models~\cite{LLFlow, jiang2024lightendiffusion,quadprior}, have surpassed traditional methods like histogram equalization~\cite{celik2011contextual, cheng2004simple} and Retinex-based approaches~\cite{li2018structure, wang2013naturalness}, they still face significant challenges. 
%
These methods can introduce artifacts or fail to restore sufficient detail in extremely dark images, which in turn limits the performance of any subsequent pose estimation model.

\noindent\textbf{Unpaired Image-to-Image Translation}
Unpaired image-to-image (I2I) translation offers a promising direction for generating synthetic training data. 
%
Seminal works like CycleGAN~\cite{CycleGAN2017} enabled translation without paired data, a concept extended by style transfer methods like AdaIN~\cite{huang2017arbitrary}. 
%
More recently, diffusion-based models~\cite{kim2023unsb,chung2024style,xia2024diffusion,xia2024diffi2i} have demonstrated powerful capabilities in domain mapping. 
%
However, the primary objective of these generic I2I methods is to alter global appearance and texture. They are not specifically designed to synthesize the complex, non-uniform noise and structural degradation characteristic of low-light conditions, which is crucial for training a robust pose estimator. 
%
This distinction motivates our work on a specialized low-light augmentation strategy tailored for high-level vision tasks.
%
\input{figures/overall_arch}




\section{Method}
\label{sec:method}
%
\noindent\textbf{Overview} 
UDAPose is a novel unsupervised domain adaptation framework that synthesizes \edit{realistic}{} low-light images from well-lit ones and adaptively fuses visual cues with learned pose priors for robust human pose estimation. 
%
As illustrated in~\cref{fig:overall_arch}, our approach uses a pre-trained Stable Diffusion (SD) model to transfer scene structure from an annotated well-lit image while injecting low-light characteristics from an unlabeled reference image, enabling supervised pose training in the low-light conditions without requiring low-light annotations. 
%
We obtain the style-infused latent code $z_0$, which embeds the structure of the well-lit image $I_\text{WL}$ and the low-frequency style of the reference $I_\text{LL}$ following~\citet{chung2024style}.
%
During the decoding process, $z_0$ is decoded, where low-light noise patterns are injected through two key modules, DHF and LCIM.
%
The diffusion backbone is responsible for preserving the scene structure and low-frequency appearance from the well-lit image, while DHF and LCIM focus on injecting high-frequency low-light characteristics.
%
The obtained low-light images are then used as training data for our Transformer-based pose estimator, where our DCA module adaptively balances image cues and pose priors to mitigate unreliable visual information under low-light conditions.


\begin{comment}

We tackle the challenge of 2D human pose estimation in low-light conditions with UDAPose, a novel unsupervised domain adaptation framework. As shown in Figure~\ref{fig:overall_arch}, UDAPose leverages a pre-trained Stable Diffusion (SD) model~\cite{latentdiffusion} to synthesize a realistic low-light image $\hat{I}_{\rm LL}$. It achieves this by combining the structural content from an annotated well-lit image $I_{\rm WL}$ with the low-light characteristics of an unlabeled low-light reference image $I_{\rm LL}$. This approach enables the direct transfer of pose annotations from $I_{\rm WL}$ to $\hat{I}_{\rm LL}$, allowing \edit{fully}{} supervised training of a pose estimator \edit{in the low-light domain}{for low-light conditions}.


Our synthesis pipeline uses the frozen VAE encoder $\mathcal{E}$, decoder $\mathcal{D}$, and UNet denoising backbone of the SD model. The process consists of three stages \edit{orchestrated}{enabled} by our novel modules:
First, to capture scene structure and low-frequency appearance, we encode the well-lit input $I_{\rm WL}$ into a latent code $z_{\rm WL} = \mathcal{E}(I_{\rm WL})$. 
%
In parallel, we encode the reference image $I_{\rm LL}$ to obtain a latent code.
%
This code modulates $z_{\rm WL}$ to produce a style-infused latent code $z_0$ following~\citet{chung2024style}. 
%
Second, to transfer high-frequency low-light noise, our Direct-Current-based High-Pass Filter (DHF) module extracts noise components from $I_{\rm LL}$ using Fast Fourier Transform (FFT).
After mean correction, the filtered outputs are encoded by $\mathcal{E}$ to obtain multi-scale high-frequency intermediate features $\{z_1, \dots, z_4\}$ that represent realistic low-light characteristics.
%
Finally, the decoder $\mathcal{D}$ generates the image $\hat{I}_{\rm LL}$ from the latent code $z_0$. During this \edit{synthesis}{process}, our novel Low-light Characteristics Injection Module (LCIM) injects the high-frequency features $\{z_1, \dots, z_4\}$ into the corresponding layers of the decoder. This ensures the faithful rendering of complex noise patterns. 


After we have synthesize low-light image $\hat{I}_{\rm LL}$, we use it for our pose model training.
%
The image is first processed with image backbone and then transformed into a series of tokens $\mathbf{F'}$ by transformer encoder.
%
Following previous work~\cite{edpose}, we initialize human and keypoint queries $\mathbf{Q}$ from $\mathbf{F'}$ and input both into stacks of Deformable Decoder Layers~\cite{deformable-detr}.
%
Within each layer, $\mathbf{Q}$ is first encoded into structured pose prior $\mathbf{Q}_{\rm pose}$ via self-attention.
%
Later, $\mathbf{Q}_{\rm pose}$ query image features $\mathbf{F'}$ via deformable cross attention, producing image cues $\mathbf{Q}_{\rm image}$.
%
We apply Dynamic Control of Attention (DCA) module to adaptively combine $\mathbf{Q}_{\rm pose}$ and $\mathbf{Q}_{\rm image}$, producing new queries $\mathbf{Q}$ for following FFN (feed-forward network) and subsequent layers.
%
At last, each token of $\mathbf{Q}$ is decoded into keypoint coordinates via a simple linear head.
\end{comment}

% \haopeng{In general, overview is a bit too long. We may want to move some details into following sections.}
% \hawk{Rewrote the overview, now just one paragraph. Commented out the old ones, which include three paragraphs. Please check the following section and see if we need to reuse some of the sentences from the old overview.}


% \noindent\textbf{Adaptive Intensity Normalization (AIN)}
% Low-light images often contain extremely low intensity values, which can cause the VAE encoder in the SD model to produce corrupted latent codes.
% %
% To address this, we apply intensity rescaling to both the real low-light reference images and the synthesized low-light outputs generated by our model.
% %
% Specifically, we first scale the input real low-light image $I_\text{LL}$ to a more suitable range using its mean $\mu_{I_\text{LL}}$:
% \begin{equation}
%     I_\text{LL}' = I_\text{LL} \times \frac{\delta}{\mu_{I_\text{LL}}}
% \end{equation}
% where $\delta = 0.449$. 
% %
% After the VAE decoder generates its output $\hat{I}'_\text{LL}$, we rescale this output to match the mean and standard deviation of the original reference low-light image $I_\text{LL}$.
% %
% This standardization and re-scaling process ensures low-light stylistic consistency and is formulated as:
% \begin{equation}
%     \hat{I}_\text{LL} = \frac{\sigma_{I_\text{LL}}}{\sigma_{\hat{I}_\text{LL}'}} (\hat{I}_\text{LL}' - \mu_{\hat{I}_\text{LL}'}) + \mu_{I_\text{LL}}
% \end{equation}
% Here, $\mu$ and $\sigma$ denote the channel-wise mean and standard deviation, respectively. 
% %
% AIN mitigates encoder collapse on low-light inputs and preserves the illumination diversity of the reference images.
%\haopeng{Remove AIN section}


\noindent\textbf{Direct-Current-based High-Pass Filter (DHF)}
% \subsection{Direct-Current-based High-Pass Filter (DHF)}
Our framework extracts high-frequency details by applying a high-pass filter in the frequency domain, yielding an image $I_{\text{HP}}$. It can be formulated as:
\begin{equation}
    I_{\text{HP}} = \text{iFFT}(\text{FFT}(I_\text{LL}) \odot \mathcal{M} )
\end{equation}
%
where $\mathcal{M}$ is a high-pass filter, and $\text{FFT}$ and $\text{iFFT}$ denote the Fast Fourier Transform and its inverse. 
%
By design, $I_{\text{HP}}$ has a mean near zero, with its pixel values representing positive (brighter) and negative (darker) deviations from the local average.
%
A critical challenge arises when preparing $I_{\text{HP}}$ for the SD encoder, which expects inputs normalized to the standard RGB $[0, 1]$ range.
%
Direct clipping of negative values leads to irreversible information loss, especially for darker details, a critical issue in low-light scenarios. 

To address this issue, we introduce a simple yet effective module, DHF.
%
The core idea is to re-center high-frequency details by aligning their distribution with the mean brightness of the original reference image, $I_\text{LL}$.
%
This process preserves the full dynamic range of the extracted details by shifting them into a perceptually meaningful range prior to normalization. 
%
Specifically, we compute the corrected high-frequency image $I_{\text{DHF}}$ as:
\begin{equation}
    I_{\text{DHF}} = I_{\text{HP}} + (\text{mean}(I_\text{LL}) - \text{mean}(I_{\text{HP}})),
\end{equation}
where $\text{mean}(\cdot)$ calculates the global channel-wise mean of an image.
%
This operation ensures that $\text{mean}(I_{\text{DHF}}) = \text{mean}(I_\text{LL})$.
%
By adjusting the negative-valued details, this process reduces information loss during the final clipping to the $[0, 1]$ range. 
%
Consequently, DHF helps preserve both bright and dark high-frequency information, enabling a richer feature representation for low-light domain adaptation.

% \subsection{Low-light Characteristic Injection Module (LCIM)}
\noindent\textbf{Low-light Characteristic Injection Module (LCIM)}
The synthesis process is finally completed in the decoding stage, which generates the low-light image $\hat{I}_{\rm LL}$.
%
A variational autoencoder (VAE) decoder $\mathcal{D}$ takes the style-infused latent code $z_0$, embedding the structure of the well-lit image $I_{\rm WL}$ and the low-frequency style of the reference low-light image $I_{\rm LL}$, and progressively upsamples it.
%
To inject high-frequency details from the reference image into the synthesized low-light output, we introduce LCIM.

After obtaining a set of high-frequency intermediate features, ${z_1,...,z_4}$ from different scales of the high-frequency image $I_\text{DHF}$ produced by DHF, LCIM processes each $z_i$ with a lightweight convolutional layer:
\begin{equation}
    \{f_1, f_2, f_3, f_4\} = \text{LCIM}(\{z_1, z_2, z_3, z_4\}),
\end{equation}

The decoder $\mathcal{D}$ is composed of 4 convolution blocks $d_1,...,d_4$ and a convolution layer $d_\text{final}$. Each processed high-frequency feature ${f_1,...,f_4}$ is injected at the end of each convolution block by adding it to the main stream:
\begin{equation}
    \hat{I}'_\text{LL} \leftarrow d_\text{final}(d_4( d_3( d_2( d_1( z_0 ) + f_1) + f_2) + f_3) + f_4)
\end{equation}

This multi-scale injection strategy guides the synthesis process to render fine-grained low-light noise at appropriate spatial resolutions.
%
Finally, to match the global stylistic appearance of the reference, we align the channel-wise mean and standard deviation of the synthesized image $\hat{I}'_{LL}$ with those of $I_{\rm LL}$ to produce our final output, $\hat{I}_{\rm LL}$.

To optimize LCIM, we freeze the encoder and decoder of the VAE, and train the module to reconstruct low-light images using a composite loss that incorporates both spatial and frequency domains:
\begin{equation}
  \mathcal{L_\mathcal{D}} = \mathcal{L}_{\text{MSE}}(I, \hat{I}) + \lambda \mathcal{L}_{\text{freq}}(I, \hat{I}),
  \label{equ:llcd_loss_revised}
\end{equation}
where $I$ is the low-light input and $\hat{I}$ is its reconstruction. The first term, $\mathcal{L}_{\text{MSE}}$, is the mean squared error, which enforces content fidelity by minimizing pixel-wise differences. The second term, $\mathcal{L}_{\text{freq}}$, is a frequency-domain loss designed to preserve fine-grained details specific to low-light conditions. 
%
The hyperparameter $\lambda$ balances the two loss terms.
%
In particular, the second loss is defined as a weighted MSE on the Fourier magnitude spectra:
\begin{equation}
  \label{eq:freq_loss_revised}
  \mathcal{L}_{\text{freq}} = \frac{1}{MN}\sum_{u=0}^{M-1} \sum_{v=0}^{N-1} \mathcal{W}(u,v) |\mathcal{F}_{I}(u,v) - \mathcal{F}_{\hat{I}}(u,v)|^{2},
\end{equation}
where $\mathcal{F}_{I}$ and $\mathcal{F}_{\hat{I}}$ are the Fourier magnitude spectra of the input and reconstructed images, respectively, and $(M,N)$ is the image resolution. The weighting function $\mathcal{W}(u,v)$ is defined as:
\begin{equation}
  \label{eq:weighting_revised}
  \mathcal{W}(u,v) = \sin{\left(\frac{\pi|2u-M|}{2M}\right)} + \sin{\left(\frac{\pi|2v-N|}{2N}\right)}.
\end{equation}
This sinusoidal weighting scheme prioritizes mid-to-high frequency components, aiming to enhance perceptual quality and retain low-light characteristics without introducing over-sharpening artifacts. 
%
Although LCIM is trained with a reconstruction objective, it operates on high-frequency components extracted from low-light images, which mainly capture noise patterns. Thus, LCIM captures transferable low-light characteristics that can be applied to synthesize low-light effects for different input images.


% \subsection{Dynamic Control of Attention (DCA)}
\noindent\textbf{Dynamic Control of Attention (DCA)}
%
\input{figures/l2norm_compare}
%
After synthesizing the low-light image $\hat{I}_\text{LL}$, we use it for our pose model training.
%
$\hat{I}_\text{LL}$ is first processed with a feature extractor and then transformed into tokens $\mathbf{F'}$ by a Transformer encoder.
%
We denote the visual tokens carrying image cues after deformable cross-attention as $\mathbf{Q}_\text{image}$ (corresponding to the output of deformable token-to-human/keypoint attention in \cite{edpose}).
%
Our pose model also initializes keypoint latents and performs self-attention among them, forming a pose-prior representation denoted as $\mathbf{Q}_\text{pose}$ (corresponding to the output of human-to-keypoint interactive attention in \cite{edpose}).
%
Within each deformable decoder layer, we need to fuse the pose prior latent $\mathbf{Q}_\text{pose}$ from self-attention and image cues latent $\mathbf{Q}_\text{image}$ from deformable cross-attention.
%
Existing DETR-based human pose estimators~\cite{edpose,grouppose,tan2024diffusionregpose} (built on~\cite{DETR,deformable-detr}) directly sum $\mathbf{Q}_\text{pose}$ and $\mathbf{Q}_\text{image}$ before the feedforward network (FFN), a rigid design that leads to degraded performance under low-light conditions.


Following the analysis framework of~\citet{elhage2021mathematical,kim2025peri}, we evaluate the ratio of Frobenius Norm of $\mathbf{Q}_\text{image}$ and $\mathbf{Q}_\text{pose}$ in typical low-light conditions that one or more human joints are barely visible under low-light conditions, as shown in~\cref{fig:l2norm-vis}.
%
When both knees are nearly indistinguishable from the background, the ratio remains approximately $1.7$, comparable to that of the clearly visible keypoints.
%
In fact, across a set of well-lit images, this ratio remains stable with a mean around $1.68$.
%
This clearly demonstrates that rigid summation fails to reduce the contribution of unreliable image cues when keypoints are barely visible, leading to incorrect pose estimation for both knees as shown in~\cref{fig:l2norm-before}.


To address this issue, we introduce DCA, which adaptively fuses the pose prior latent $\mathbf{Q}_\text{pose}$ from self-attention and image cues latent $\mathbf{Q}_\text{image}$ from deformable cross-attention.
%
DCA first concatenates $\mathbf{Q}_\text{pose}$ and $\mathbf{Q}_\text{image}$ in channel dimension as $\mathbf{Q}_\text{cat}$,
\begin{equation}
\mathbf{Q}_\text{cat} = \text{Concat}(\mathbf{Q}_\text{pose}, \mathbf{Q}_\text{image}).
\end{equation}
%
Then, $\mathbf{Q}_\text{cat}$ is fed into a two-layer MLP that reduces the channel dimension to two.
%
A softmax function is then applied to produce two competitive weights corresponding to the pose-prior and image-cue features,
\begin{equation}
(\mathbf{w}_\text{pose}, \mathbf{w}_\text{image}) = \text{softmax}(\text{MLP} (\mathbf{Q}_\text{cat})).
\end{equation}
%
where $\mathbf{w}_\text{pose}$ and $\mathbf{w}_\text{image}$ are the obtained weights for $\mathbf{Q}_\text{pose}$ and $\mathbf{Q}_\text{image}$.
We then apply Hadamard product of the weights and their corresponding latent, where the new queries $\mathbf{Q}$ for the subsequent FFN and following layers are obtained by a weighted sum of $\mathbf{Q}_\text{pose}$ and $\mathbf{Q}_\text{image}$,
\begin{equation}
\mathbf{Q} = \mathbf{w}_\text{pose} \odot \mathbf{Q}_\text{pose} \oplus \mathbf{w}_\text{image} \odot \mathbf{Q}_\text{image}.
\end{equation}
%
Notably, DCA assigns different weights for different keypoints of a human instance, allowing the model to rely more on pose priors when a keypoint is less visible, and more on image cues when a keypoint is visible.
%
With only two additional linear layers, DCA enables the model to balance the influence of image cues and pose prior, leading to improved performance under low-light conditions as shown in~\cref{fig:l2norm-vis,fig:l2norm-after}.


\noindent\textbf{Pose Estimation Training}
% \subsection{Pose Estimation Training}
%
For the human pose estimation model, we adopt the loss formulation from ED-Pose~\cite{edpose}. We employ a set-based Hungarian loss that forces
a unique prediction for each ground-truth box and keypoint. The total loss is a weighted sum of classification $\mathcal{L}_c$, human box regression $\mathcal{L}_h$, and keypoint regression loss $\mathcal{L}_k$. Notably, $\mathcal{L}_k$ simply
consists of the normal L1 loss and the constrained L1 loss named Object Keypoint Similarity (OKS) loss~\cite{rw-petr} without any dense supervision (e.g., heatmap). Please refer to the supplementary material for details.

% \begin{equation}
%   \mathcal{L}_{\text{pose}} = \mathcal{L}_{\text{heatmap}} + \gamma \mathcal{L}_{\text{offset}}.
% \end{equation}




\section{Experiment}
\label{sec:exp}
%
% \subsection{Implementations and dataset}
% We provide more details in supplementary.


\noindent\textbf{Datasets}
We evaluate UDAPose on the ExLPose dataset~\cite{ExLPose_2023_CVPR}, specifically designed for benchmarking 2D human pose estimation in extremely low-light conditions.
%
% \edit{The ExLPose training set consists of 2,065 well-lit and optically filtered low-light image pairs, with pose annotations following the CrowdPose format.
% %
% These images span 251 indoor and outdoor scenes, with low-light versions generated using a dual-camera system under varying conditions to simulate diverse low-light scenarios. }{}
ExLPose provides two distinct test sets: ExLPose-OCN and ExLPose-test.
%
ExLPose-OCN contains 360 real low-light images captured at night using A7M3 and RICOH3 cameras.
%
ExLPose-test consists of 491 optically filtered images, where brightness is reduced by a factor of 100.
%
ExLPose-test, also referred to as Low-Light All (LL-A), is further divided into three difficulty levels: Low-Light Normal (LL-N), Low-Light Hard (LL-H), and Low-Light Extreme (LL-E).


To validate our method's generalization ability, we performed cross-dataset evaluation on EHPT-XC~\cite{ehpt-xc}.
%
EHPT-XC is a novel hybrid dataset combining RGB and event data, specifically designed for human pose estimation and tracking in challenging low-light and motion blur conditions.
%
% \edit{
% It encompasses RGB video frames from 158 diverse sequences, along with pixel-wise aligned and temporally synchronized event streams, and annotations containing 38K 2D keypoints and bounding boxes with track IDs.}{}
%
Given that some RGB data in EHPT-XC primarily exhibits motion blur without low-light conditions, we combined the train and test split of EHPT-XC and selected a specific subset of 12 scenes (1200 images) under low-light conditions for cross-dataset evaluation.
%
% \edit{This subset allows us to assess method performance under unseen low-light scenarios.}{}

\input{tables/tab_exlpose-test-AP}


\noindent\textbf{Evaluation metrics}
%
% Our evaluation follows the COCO protocol~\cite{dataset-coco}, as used in LSBN+LUPI~\cite{ExLPose_2023_CVPR}, for testing on both the ExLPose-test and ExLPose-OCN datasets.
We evaluate our method following the COCO evaluation protocol~\cite{lin2014microsoft}, consistent with exisiting methods~\cite{ExLPose_2023_CVPR,ella-eccv, ehpt-xc}, on ExLPose-test, ExLPose-OCN, and EHPT-XC.
%
% For each subset, we report Average Precision across multiple thresholds (i.e., AP@0.5:0.95) as the performance metric.
For each subset, we report Average Precision (AP) and Average Recall (AR) across multiple thresholds (@0.5:0.95) as the primary performance metrics.


\noindent\textbf{Implementation details}
%
We adopt SD-2.1-base as our backbone model for low-light data synthesis.
%
During training data synthesis, we use DDIM~\cite{song2020ddim} as our solver and 50 steps in sampling process.
%
% \edit{For training LICM, we combine ExLPose-test low-light images and ExLPose-OCN images as our unlabeled low-light dataset while keeping the encoder parameters frozen. Our training process involves randomly cropping images to $512 \times 512$ pixels and applying random flipping for data augmentation.}{}
%
We train LCIM using Adam optimizer~\cite{kingma2014adam} over 400
epochs in total, with an initial learning rate of $4 \times 10^{-6}$ that decreases
to $4 \times 10^{-7}$ after 300 epochs.
%
We train with a batch size of 32 across 4 NVIDIA RTX4090 GPUs and set the
weight $\lambda$ in~\cref{equ:llcd_loss_revised} to $4 \times 10^{-4}$ during training
%
% Our framework uses DEKR-W32~\cite{DEKR2021} as the backbone for the human pose estimation model to ensure a fair comparison with the recent low-light human pose estimation approach ELLA~\cite{ella-eccv}.
%
Our framework uses ED-Pose~\cite{edpose} with Swin-T~\cite{liu2021swin} pretrained on ImageNet 22k~\cite{deng2009imagenet} as the backbone for the human pose estimation model.
%
Training is performed with a batch size of 16 on 2 NVIDIA RTX PRO 6000 Blackwell GPUs.
%
% \edit{During training, we resize input images to $512 \times 512$ and apply data augmentations following DEKR, including random rotation ($\pm30^\circ$), scaling (0.75–1.5×), translation ($\pm40$ pixels), and flipping. We adopt the same training strategy as DEKR, with the only modification being the loss weighting factor $\gamma = 0.03$.}{}

% \noindent
% \textbf{Baselines } For comparative evaluation, we benchmark against state-of-the-art
% and highly cited methods in two categories: image enhancement (RFormer, LLFlow
% and QuadPrior~\cite{cai2023retinexformer,LLFlow,quadprior}) and domain adaptation
% (UDA-HE, AdvEnt, CycleGAN, UNIT, UNSB~\cite{CycleGAN2017,UNIT,kim2023unsb,AdvEnt,kim2022unified}).
% We also include ELLA~\cite{ella-eccv}, the current SOTA method for low-light human
% pose estimation, in our comparison.
% %
% To establish a fair comparison framework, we utilize the same base human pose
% estimator, DEKR~\cite{DEKR2021}, across all methods including our own.
% %
% Following ExLPose's~\cite{ExLPose_2023_CVPR} methodology, we modified AdvEnt~\cite{AdvEnt}
% by replacing its semantic segmentation backbone with our 2D pose estimator.
% %
% For UDA-HE~\cite{kim2022unified}, which originally operates as a model-agnostic
% domain-adaptive human pose estimation method, we upgraded its ResNet backbone to
% HRNet (matching our method's backbone) and retrained the AdaIN component to ensure
% equitable comparison.
% %
% It's worth noting that UDA-HE employs a bottom-up paradigm.
% %
% We also compare our framework to ELLA~\cite{ella-eccv}, the SOTA method of low-light
% human pose estimation.
% %
% Note that we have the same pose model settings as the main teacher and student in
% ELLA~\cite{ella-eccv}. However, the student model in ELLA distillates from dual teachers.
% %
% As our work main focus on data synthesis, we do not conflict with the teacher-student
% framework.
% %
% For fairness, our pose model training is well-aligned with the main teacher training
% and compare to it.
% %
% We discuss the the comparison to the full model proposed in ELLA~\cite{ella-eccv}
% in Supplementary.


% For domain-adaptive baselines, we modify AdvEnt~\cite{AdvEnt} following ExLPose~\cite{ExLPose_2023_CVPR} by replacing its semantic segmentation backbone with our 2D pose estimator. Similarly, UDA-HE~\cite{kim2022unified}, originally designed as a model-agnostic approach, is adapted by upgrading its ResNet backbone to HRNet (matching our model) and retraining its AdaIN module to ensure consistency. 

\noindent\textbf{Baselines} For comparative evaluation, we benchmark against state-of-the-art methods in two categories: image enhancement (RFormer, DarkIR, QuadPrior, and LightenDiff~\citep{cai2023retinexformer,feijoo2025darkir,quadprior,jiang2024lightendiffusion}) and domain adaptation (CycleGAN, UNIT, UDA-HE, UNSB, EnCo~\citep{CycleGAN2017,UNIT,kim2022unified,kim2023unsb,cai2024enco}).
%
We also include ELLA~\cite{ella-eccv}, the state-of-the-art (SOTA) method for low-light human pose estimation.
%
To ensure a fair comparison, we use ED-Pose~\cite{edpose} as the backbone network across all methods, including our own.
%
While ELLA~\cite{ella-eccv} adopts a dual-teacher-student framework, where the student model distillates from dual teachers utilizing low-light images, our method instead focuses on low-light synthesis and balancing pose priors and visual cues.
% {This sentence is wrong? Using low-light training images?}
% \haopeng{Not precise enough. In knowledge acquisition stage, student would utilize degraded real LL (from ExLPose LL dataset) with pseudo labels from teachers for training.} 
%
To evaluate the performance of data synthesis, the low-light data augmentation part of ELLA is applied in the comparison.
%
A full comparison to ELLA’s complete dual-teacher-student framework is provided in the supplementary material.
%
% \edit{To show the effectiveness and necessity of our method, we also include zero-shot performance from Sapiens. Note that as Sapiens is a top-down method, we directly use the ground-truth bounding box to crop out single human instance as input, leading to extra advantages compared to other baselines and our pose model. As QuadPrior is a source-free method, we directly use authors' provided checkpoint trained on COCO to have best performance. Also, LightenDiff requires pair images in different illumination level to train, which is not feasible in ExLPose dataset. We also use authors' provided checkpoint to have best performance.}{}


\subsection{Performance on ExLPose-test}
%
%
\input{tables/tab_exlpose-test-AR}
%
As shown in~\cref{tab:exlpose-test-AP,tab:exlpose-test-AR}, UDAPose consistently outperforms all baselines on the ExLPose-test set. On average across all low-light conditions (LL-A), UDAPose achieves 27.0 AP and 36.5 AR, surpassing the strongest baseline, CycleGAN~\cite{CycleGAN2017} and ELLA~\cite{ella-eccv}, by 7.4 AP (a 37.8\% relative improvement) and 7.6 AR (a 26.3\% relative improvement), respectively. 
%
The performance gap widens as lighting conditions deteriorate. Specifically, UDAPose leads by 5.0 AP and 2.6 AR on the normal subset (LL-N) and by 10.1 AP (a 56.4\% relative gain) and 9.4 AR (a 33.6\% relative gain) on the hard subset (LL-H).
%
The advantage is clearest on the extreme subset (LL-E), where UDAPose delivers a more than three-fold improvement over ELLA on AP (11.7 vs. 3.4 AP) and more than double on AR (20.4 vs. 9.7 AR). Our method outperforms all baselines across diverse low-light conditions.


\subsubsection{Qualitative Analysis}
%
\input{figures/representative_result}
%
\cref{fig:qualitative} provides a qualitative comparison against representative methods. In normal low-light conditions, UDAPose already yields more precise joint localization. As lighting degrades, our superiority becomes more evident. 
%
In hard low-light, competing methods produce poses with significant limb errors, whereas UDAPose maintains an accurate skeletal structure. Under extreme low-light, where the subject is barely visible, other methods generate fragmented and anatomically implausible poses. In contrast, UDAPose successfully reconstructs a complete and coherent human pose. These visual results support our quantitative findings, confirming that our synthetic data generation and adaptive fusion of learned pose priors and image cues enable robust pose estimation in challenging low-light scenarios.




\subsection{Performance on ExLPose-OCN}
\input{tables/tab_exlpose-ocn}
%
\cref{tab:exlpose-ocn} presents our quantitative results on the ExLPose-OCN dataset. Our model achieves an average AP of 51.4 and an average AR of 65.1, a 5.4 AP improvement (11.7\% relative gain) and a 2.8 AR improvement (4.5\% relative gain) over the previous state-of-the-art~\cite{ella-eccv}. 
% %
% While our method surpasses most baselines, Sapiens~\cite{khirodkar2024sapiens} also performs well. 
% %
% We attribute this to the nature of the OCN dataset, which often contains localized light sources that illuminate some joints while obscuring others. 
% %
% Sapiens' extensive pre-training and ability to handle occlusions make it well-suited for these partially visible scenarios.
% To further explore the impact of a strong well-lit pose foundation, we introduce a variant, ``Ours (CrowdPose)''. This model is first pre-trained on the large-scale CrowdPose dataset~\cite{li2019crowdpose} and then adapted using our synthetic low-light data. 
% %
% This pre-training strategy alone improves performance by about 12 AP, resulting in a final average AP of 48.4. 
% %
% Crucially, this enhanced model significantly outperforms Sapiens by 7.8 AP and 8.8 AP on the A7M3 and RICOH3 subsets, respectively. 
% %
% This is especially notable given that Sapiens is trained on a much larger dataset and requires ground-truth bounding boxes, an advantage our bottom-up method does not have.  
%
These results show that our approach enables robust pose estimation in real-world low-light conditions where annotated data is scarce.

\input{tables/tab_zero-shot}

\input{tables/tab_abl}

\subsection{Cross-dataset validation on EHPT-XC}
%
To assess our model's generalization ability, we perform a cross-dataset validation on the EHPT-XC dataset~\cite{ehpt-xc}, which features challenging real-world conditions such as motion blur and low light.
%
As shown in~\cref{tab:zero-shot}, our method consistently outperforms all state-of-the-art baselines across all Average Precision (AP) and Average Recall (AR) metrics.
%
Specifically, our approach achieves an AP@0.5:0.95 of 31.0, surpassing the strongest baseline, ELLA~\cite{ella-eccv}, by 7.4 points.
%
This strong performance also extends to other metrics, highlighting our model’s ability to generalize to unseen and degraded data without fine-tuning.


% \subsubsection{Analysis of Key Components}
% As shown in Table~\ref{tab:abl}, we incrementally add our proposed modules to a baseline model to demonstrate their effectiveness.


\subsection{Ablation Studies}




\subsubsection{Baselines}
We first establish two baselines. A standard pose estimator trained only on well-lit data fails on low-light images (e.g., 3.4 AP on LL-N), highlighting a significant domain gap. 
Adapting this model with a simple histogram matching technique offers only a marginal improvement (21.3 AP on LL-N), indicating that basic color transformations are insufficient. 
A second baseline, ``Baseline SD'', following~\citet{chung2024style}, achieves descent performance by synthesizing low-light images (23.7 AP on LL-N) but still struggles with more challenging conditions (7.2 AP on LL-H).

\subsubsection{Component Analysis}
As shown in~\cref{tab:abl}, building on ``Baseline SD'', we first integrate LCIM, which yields the most substantial performance leap. The LCIM dramatically improves results on the most difficult subsets, increasing the AP on LL-H from 7.2 to 20.7 and on LL-E from 0.0 to 7.8.
%
This highlights the importance of LCIM in transferring low-light features from the reference image.
%
\edit{To further enhance realism we add DHF module.
This module consistently}{In addition, the DHF module} improves performance by modeling frequency-domain attributes, delivering notable performance gains on challenging data (LL-H: +4.6 AP, LL-E: +1.6 AP).
%
Lastly, DCA is added to improve our pose model's capability to deal with low-visibility conditions, leading to consistent improvement across all subsets, from LL-N (+3.4 AP) to more \edit{challenge}{challenging} LL-H (+2.7 AP) and LL-E (+2.3 AP).
%
Overall, each component plays a clear role, and together they improve the model’s ability to handle varied low-light scenarios.
% \subsubsection{Full Model}
% Finally, our ``Pair-guided'' training strategy further optimizes the framework. 
% %
% While it involves a minor performance trade-off on some subsets (e.g., -0.8 AP on LL-H), it improves performance on well-lit data (+1.2 AP on WL) and achieves the best overall results.
% More importantly, this strategy streamlines the training process into a single, efficient stage. 
% %


\input{tables/tab_abl-skip}

\subsubsection{Analysis of LCIM}
\label{sec:ablation_skips}
We now analyze the core of our LCIM module: the multi-scale intermediate features. As detailed in~\cref{tab:abl-skip}, we start with a baseline model ($z_0$) that omits all intermediate features, then progressively integrate features from coarse to fine levels ($z_1$ to $z_4$). 
The $z_0$ model, achieves a modest 40.0 AP on A7M3 and 36.8 AP on RICOH3.

These results show that fusing multi-scale features is important. 
%
Each added intermediate feature brings a consistent performance improvement. 
%
Adding all four feature levels ($+z_1+z_2+z_3+z_4$) results in our strongest model, improving the AP by +15.0 on A7M3 (40.0$\rightarrow$55.0) and +11.1 on RICOH3 (36.8$\rightarrow$47.9) compared to the $z_0$ baseline. 
%
This analysis shows that our coarse-to-fine fusion strategy effectively uses multi-scale latent features from the SD encoder, which is important for robust pose estimation under challenging low-light conditions.




% \subsection{Anatomical Consistency}
% \haopeng{Consider move to supp.}
% %
% \input{tables/tab_consistency}
% %
% We evaluate the anatomical consistency of our generated low-light images, a critical factor for reusing pose annotations from well-lit images.
% %
% To this end, we synthesize low-light images from the ExLPose dataset and compare them against ground-truth images using a comprehensive set of metrics.
% %
% We assess image fidelity at the pixel level with PSNR and SSIM, and at the feature level with LPIPS and Fr\'echet Inception Distance (FID).
% %
% More importantly, to directly quantify anatomical integrity, we compute the Kullback–Leibler (KL) divergence between pose keypoint heatmaps. These heatmaps are inferred by a pre-trained pose estimator from our synthetic images versus the ground-truth images.

% As presented in Table~\ref{tab:consistency}, our method significantly outperforms all baselines across every metric.
% %
% It achieves a PSNR of 41.13 and an SSIM of 0.91, indicating superior pixel-level accuracy.
% %
% Furthermore, our method obtains the lowest LPIPS (0.20) and a remarkably low FID of 11.17, confirming that the generated images have higher perceptual quality and a feature distribution much closer to that of real images.
% %
% Crucially, our method yields a KL divergence of only 0.008, which is an order of magnitude lower than the best-performing baseline (CycleGAN: 0.028). This result provides direct evidence that our generation process preserves the underlying human anatomical structure with high precision.
% %
% Consequently, the pose information extracted from our synthetic data is nearly identical to that from real low-light images, validating our method's effectiveness for downstream pose estimation tasks.





% \subsection{Qualitative results}
% \haopeng{Move to supp.}
% qualitative comparison
% \input{figures/qualitative}
%
% We present a qualitative comparison between our UDAPose framework and existing methods in \cref{fig:gen-result-comp}. 
% %
% The visual results clearly demonstrate the superior capability of our approach in generating realistic low-light images that closely resemble the real low-light ground truth.

% Examining the enhancement-based method, QuadPrior~\cite{quadprior} attempts to brighten low-light images but tends to produce over-smoothed results with significant loss of texture and detail.
% %
% Among image-to-image translation methods, CycleGAN~\cite{CycleGAN2017} produces images with excessive color shifts and unrealistic noise patterns. 
% %
% UNIT~\cite{UNIT} and UNSB~\cite{kim2023unsb} generate images with irregular noise distributions that significantly differ from real low-light conditions, making them less effective for training robust pose estimation models. 
% %
% StyleID~\cite{chung2024style}, while better at preserving the overall scene structure, still struggles to accurately capture the complex noise patterns characteristic of low-light photography.

% In contrast, our UDAPose framework generates low-light images that exhibit remarkably realistic noise characteristics. 
% %
% The synthetic images produced by our method faithfully preserve essential high-frequency details while accurately modeling the complex noise patterns present in real low-light conditions. 
% %
% The superior quality of our synthetic low-light images can be attributed to the CIM module, which effectively captures and transfers the complex low-light characteristics from unpaired real low-light images to well-lit inputs. 
% %
% By leveraging Stable Diffusion's generative capabilities combined with our CIM, UDAPose overcomes the limitations of previous approaches, generating more realistic training data that better prepares the pose estimation model for real-world low-light scenarios.
% We present a qualitative comparison of UDAPose against existing methods in Figure~\ref{fig:gen-result-comp}, demonstrating its superior ability to generate realistic low-light images that closely resemble real low-light ground truth.

% For enhancement-based methods, QuadPrior~\cite{quadprior} brightens low-light images but produces over-smoothed results, leading to a loss of texture and fine details. Among image-to-image translation approaches, CycleGAN~\cite{CycleGAN2017} introduces excessive color shifts and unrealistic noise patterns, while UNIT~\cite{UNIT} and UNSB~\cite{kim2023unsb} generate irregular noise distributions that fail to match real low-light characteristics, making them less effective for training pose estimation models. StyleID~\cite{chung2024style} better preserves scene structure but still struggles to capture the complex noise patterns inherent to low-light conditions.

% In contrast, UDAPose generates synthetic low-light images that exhibit realistic noise characteristics and faithfully preserve essential high-frequency details. The improvements stem from our LCIM module, which effectively captures and transfers complex low-light characteristics from unpaired real low-light images to well-lit inputs. By integrating Stable Diffusion’s generative capabilities with LCIM, UDAPose overcomes the limitations of prior methods, producing high-quality synthetic training data that significantly enhances pose estimation in real-world low-light scenarios. We provide more qualitative results and further discussion in the supplementary material.




\section{Conclusion}
\label{sec:con}
%
In this work, we introduced UDAPose, a novel domain-adaptive framework for human pose estimation under low-light conditions.
%
UDAPose leverages SD to synthesize \edit{realistic}{} low-light images, incorporating the DHF with LCIM to retain key low-light details.
%
UDAPose also integrates DCA to balance unreliable visual cues under poor illuminated conditions with learned pose priors. 
%
This results in improved performance under extreme lighting conditions.
%
Our approach outperforms both rule-based and learning-based augmentation methods, achieving substantial performance gains on ExLPose and EHPT-XC.
%
These results demonstrate UDAPose’s effectiveness in addressing limitations of existing low-light human pose estimation methods and improving human pose estimation performance in real-world low-visibility scenarios.



==> tables/rebuttal/tab_control.tex <==
\vspace{-0.25cm}
\begin{table}[h]
%
\fontsize{6pt}{7pt}\selectfont % Set font size to 9pt with 11pt baselineskip
\setlength{\tabcolsep}{1mm} % Reduce horizontal space between columns to 1mm
\centering
    \begin{tabular}{l| c | rrr | cc | c}
    \hline
    \hline
          & \multicolumn{7}{c}{\textbf{AP$^{\uparrow}$@{0.5:0.95}}} \\
    \cline{2-8}            &  WL  & LL-N & LL-H & LL-E & A7M3 & RICOH3 & EHPT-XC \\
    \hline
    ControlNet   & 66.3 & 31.7 & 16.4 & 2.7 & 47.6 & 43.7 & 22.4  \\
    IP-Adapter  & 65.8 & 31.5 & 17.1 & 3.5 & 48.4 & 43.4 & 24.1  \\
    \hline
    Baseline SD + AIN      & 60.1 & 25.2 & 8.8 & 2.4 & 33.0 & 27.8 & 6.1  \\
    \hline
    SE-Block     & 62.4 & 36.7 & 26.3 & 9.5 & 50.3 & 46.5 & 26.7  \\
    CBAM         & 62.5 & 37.0 & 26.2 & 9.8 & 51.1 & 46.2 & 27.0  \\
    \hline
    Ours (ExLPose)         & 67.3 & 38.7 & 28.0 & 11.7 & 55.0 & 47.9 & 31.0  \\
    Ours (CrowdPose)         & 71.7 & 47.9 & 37.2 & 19.4 & 70.5 & 69.7 & 45.7  \\

    \hline
    \hline
  \end{tabular}
  %
  \centering
  \vspace{-0.3cm}
  \caption{
    Performance comparison across baselines, design alternatives, and dataset  scaling evaluation.
  }
  \label{tab:control}
\end{table}
\vspace{-0.35cm}

==> tables/rebuttal/tab_lambda.tex <==
\begin{table}[!t]
%
\fontsize{7pt}{8pt}\selectfont % Set font size to 9pt with 11pt baselineskip
\setlength{\tabcolsep}{1.2mm} % Reduce horizontal space between columns to 1mm
\centering
    \begin{tabular}{l|cc|cc|c}
    \hline
    \hline
    \textbf{Value}  & \textbf{PSNR}$^{\uparrow}$ & \textbf{SSIM}$^{\uparrow}$ & \textbf{LPIPS}$^{\downarrow}$ & \textbf{FID}$^{\downarrow}$ & \textbf{KL}$^{\downarrow}$ \\
    \hline
    % Paired low-light     &     $\infty$    &     1.000     &      0.000     &             \\
    % \hline
    aa  & 36.56 & 0.76 & 0.26 & 50.20 & 0.028  \\
    bb  & 33.90 & 0.66 & 0.29 & 45.70 & 0.104  \\
    cc  & 34.19 & 0.74 & 0.30 & 96.42 & 0.062  \\
    dd  & 35.99 & 0.75 & 0.28 & 48.71 & 0.031  \\
    \hline
    \hline
    \end{tabular}
%
\centering
\caption{
    Caption of Table 3
}
%
\label{tab:lambda}
\end{table}

==> tables/rebuttal/tab_mask.tex <==
\begin{table}[!t]
%
\fontsize{7pt}{8pt}\selectfont % Set font size to 9pt with 11pt baselineskip
\setlength{\tabcolsep}{1.2mm} % Reduce horizontal space between columns to 1mm
\centering
    \begin{tabular}{rrrrrr}
    \hline
    \hline
    \multicolumn{6}{c}{\textbf{AP$^{\uparrow}$@{0.5:0.95}}} \\
    \hline
    2 & 4 & 6 & 8 & 10 & 12 \\
    \hline
    xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
    

    \hline
    \hline
  \end{tabular}
  %
  \centering
  \caption{
    Caption of Table 4. \haopeng{Probably we don't want to use a table for this question.}
  }
  \label{tab:mask}
\end{table}

==> tables/tab_cross.tex <==
\begin{table}[!t]
%
\fontsize{9pt}{10pt}\selectfont % Set font size to 9pt with 11pt baselineskip
\setlength{\tabcolsep}{1.2mm} % Reduce horizontal space between columns to 1mm
\centering
\resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{l|cc|cccc|cc}
    \hline
    \hline
    \multirow{2}{*}{\textbf{Methods}}            & \multicolumn{6}{c}{\textbf{AP$^{\uparrow}$@0.5:0.95}} \\ 
                                                                     \cline{2-9} 
                                                                     &CrowdPose&  WL  & LL-A & LL-N & LL-H & LL-E & A7M3 & RICOH3 \\ 
    \hline
    Sapiens~\cite{khirodkar2024sapiens}~\scriptsize({ECCV})          &   49.7  & 53.3 &  6.1 & 14.4 &  1.5 &  0.0 & 41.8 &  38.4  \\
    \hline
    CrowdPose                                                        &   66.0  & 60.2 &  3.4 &  7.9 &  0.8 &  0.2 & 22.8 &  27.8  \\
    +Synthetic                                                       &   64.5  & 59.8 & 22.1 & 33.6 & 22.0 &  6.8 & 49.6 &  47.2  \\
    \hline
    \hline
    \end{tabular}
}
%
\centering
\caption{
    Zero-shot generalization using Sapiens~\cite{khirodkar2024sapiens}. Training on CrowdPose and with our synthetic low-light images.
}
%
\label{tab:cross}
\end{table}
